Pay for a Sliding Bloom Filter and Get Counting, Distinct Elements, and Entropy for Free

For many networking applications, recent data is more significant than older data, motivating the need for sliding window solutions. Various capabilities, such as DDoS detection and load balancing, require insights about multiple metrics including Bloom filters, per-flow counting, count distinct and entropy estimation. In this work, we present a unified construction that solves all the above problems in the sliding window model. Our single solution offers a better space to accuracy tradeoff than the state-of-the-art for each of these individual problems! We show this both analytically and by running multiple real Internet backbone and datacenter packet traces.

==> OVS_graphs/ovseval.tex <==

\section{Open vSwitch Implementation}
Next, we evaluate a prototype implementation of the proposed HHH algorithms in OVS. We first provide an overview of OVS architecture. Then, we dive into how HHH are implemented in OVS and on its performance.

\input{ovsOverview}

\subsection{Implementation Design}
We implement HHH algorithms as part of the dataplane ... 

%The first uses Skipper as a dynamic sampling technique and performs the measurement in a separate virtual machine that can be placed anywhere in the cloud.
%A second option is to perform the measurement itself inside of the data plane as an integral path of the datapath.
%This alternative yields higher throughput as data is transmitted to the measurement VNF. However, this alternative creates coupling between the measurement algorithm and the virtual switch.
%These options are illustrated in Figure~\ref{fig:dut}.

%implementation where network monitoring is an integral part of the tasks performed by the datapath. 

%That is, it provides the capability to dynamically adjust the sample interval, the sampled packets are then forwarded to a virtual machine that contains the measurement algorithm. This implementation offers more flexibility, and is in line with the NFV paradigm. The drawback of this implementation are the additional overheads that are imposed by switching traffic toward a separate VNF.  
 
%It is important to note that, while our implementation deal to DPDK-accelerated datapath, they can easily be adopted to other versions. 

%Second, we consider that the back box HH algorithm (in our case SSH) is running apart of OVS. This particular design is essential to understand and assess since decoupling network functionalities (in this case, the monitoring) is one of the main advantages and premises of NFV. 
%
%For this implementation, we basically forward packets to the black box VNF according to the adaptive update probability. Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are just dropped.


%Our Skipper implementation extends the DPDK accelerated datapath capabilities, it is very local and only touch the dpif component, in Figure \ref{fig:ovs}. As packets are processed through the datapath, we retain easy access to the packet metadata.  Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are dropped. Hence, our core implementation is simple and only requires few lines of code in dpif-netdev. Although our implementation is tailored to DPDK-accelerated user space datapath, its implementation on kernel versions is straightforward.



\subsection{Evaluation}
\subsubsection{Environment setup}

Our evaluation settings consist of two identical HP ProLiant servers with an Intel Xeon E3-1220v2 processor running at 3.1 Ghz with 8 GB RAM. Both servers are equipped with DPDK-enabled network interface cards (Intel 82599ES 10 Gbit/s). Each server is directly interconneced through a different physical interface. The servers run CentOS 7.2.1511 with Linux kernel 3.10.0. 

We use one server as \emph{Design Under Test (DUT)}, and the other as a traffic generator. In our \emph{DUT}, we use Open vSwitch 2.5 compiled with Intel DPDK 2.02. NIC physical ports are attached to OVS using \emph{dpdk} ports. OVS is configured so as all incoming network traffic is forwarded to another interface. In the traffic generator, we rely on the MoonGen traffic generator~\cite{MoonGen2015} tool to generate traffic at line rate. We generate UDP network traffic according to dataset Chicago16. We keep the source and destination IP prefixes as they are in the dataset and adjust the payload size in order to generate packets of 64 Bytes (reaching up to 14.88 Mpps in 10 Gbit/s NICs).

%MoonGen sends packets through one network interface and receives them on the other one after being processed by OVS.


%Scenario
%\subsubsection{Alternative Solutions}
%We evaluate the OVS performance considering the implementation of HHH algorithms.  We compare the performance of OVS without running any HHH algorithm (baseline) against our proposed solutions (RHHH and FRHHH). We compare them to Partial Ancestry implementation.

% as part of the OVS dataplane. All implementations consider the 2D Byte version. We also compare them against the case where OVS samples the packets to a third-party VNF that implements HHH algorithms. 


\begin{figure}[t]\centering
	\includegraphics[width = \columnwidth, height=5cm]{graph1.pdf}
	\caption{Measured throughput using different HHH implementations.}
	\label{fig-bw1}
\end{figure}

\begin{figure}[t]\centering
	\includegraphics[width = \columnwidth, heigInht=5cm]{graph2.pdf}
	\caption{Measured throughput of FRHHH using different filter probabilities.}
	\label{fig-bw2}
\end{figure}

\subsubsection{Results}
Figure \ref{fig-bw1} illustrates the throughput of OVS when running HHH algorithm in dataplane. For the evaluations, we consider $\epsilon = 2^10$. We compare our proposal solutions (RHHH and FRHHH) against OVS (without any HHH) and with Partial Ancestry algorithm. Observe that Partial Ancestry algorithm leads to an overhead in terms of throughput greater than 60\% in comparison to OVS baseline. In contrast, our proposal, FRHHH, leads to a negligeable throughput overhead (lower than 3\%).% , while RHHH to $~20\%$.

In Figure \ref{fig-bw2}, we illustrate the impact of different filter probabilities on the overhead of FRHHH method. Observe that as we increase the probability to update HHH, the throughput overhead increases (up to 25\%) since more packets update the HHH data structures. Observe that there is a tradeoff between the error and the achieved performance.
%
Additionally, we also compare FRHHH to the scenario which packets are sampled to a monitoring VNF. In this particular case, we assume that the VNF has an implementation of HHH. Then, OVS is required to forward a percentage of packets to that VNF. As OVS does not support natively sampling packets in the dataplane, we implement a packet uniform sampling method in the dataplane so as OVS also forwards packets to a virtual port (attached to the VNF). Observe, in Figure \ref{fig-bw2}, that considering a probability of 10\% on sampling the packets, higher penalties are obtained than doing it for 30\% of the packets in the dataplane. 


%Figure \ref{fig-bw} shows the average end-to-end throughput on the SanJose14 trace for our two designs. Similar results were obtained when running different network traces.
%As shown, measuring the data inside the data plane is efficient and reduces the throughput by only $3\%$. 
%When the measurement takes place in a dedicated VNF, Skipper increases the OVS throughput by about $25\%$.
%When the measurement is done as a part of the datapath its overheads are almost negligible and the throughput impact is less than $3\%$. The reason for that is that less traffic is routed. Alternatively, when Skipper is implemented as a VNF, the measurement reduces throughput by $13\%$, when compared to not performing measurement. Since sketches and counter based algorithms process all packets in the stream, implementing them as VNFs has higher overheads, and degrades performance by more than $30\%$. 


%We clearly observe the existence of a tradeoff between flexibility and performance between the two proposed designs. Running the monitoring HH algorithm outside OVS (in a VNF) introduces higher flexibility in the implementations of new HH strategies. In turn, compiling HH algorithm as part of the OVS datapath reduce the burden of forwarding packets to a VNF.
%




==> acc-cov.tex <==
\newcommand{\fourFigWidth}{4.2cm}
\newcommand{\thirdFigWidth}{5.47cm}
\newcommand{\twoFigWidth}{8.2cm}
%\floatplacement{figure}{H}
\begin{figure*}[t]
	\captionsetup{justification=centering}
	\begin{tabular}{cccc}
		\subfloat[Chicago15\label{ACC:CH15:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth ]
			{CH15_2Dbytes_acc.png}}  &
		\subfloat[Chicago16\label{ACC:CH16:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{CH16_2Dbytes_acc.png}}  &
		\subfloat[SanJose13\label{ACC:SJ13:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{SJ13_2Dbytes_acc.png}}  &
		\subfloat[SanJose14\label{ACC:SJ14:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{SJ14_2Dbytes_acc.png}}  	
	\end{tabular}
	\caption{	\label{fig:acc} Accuracy error ratio -- HHH candidates whose frequency estimation error is larger than $N\epsilon$ ($\epsilon =0.001$).}		
%\end{figure*}	
%\thisfloatsetup{subfloatrowsep=qquad}
%\begin{figure*}[h]	
	\captionsetup{justification=centering}
	\begin{tabular}{cccc}
		\multicolumn{4}{c}{\subfloat{\includegraphics[width = 7cm, height=0.6cm]
				{ACCCOVLegend.png}}}
		\tabularnewline
		\addtocounter{subfigure}{-1}
		\subfloat[Chicago15\label{COV:CH15:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{CH15_2Dbytes_cov.png}}  &
		\subfloat[Chicago16\label{COV:CH16:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{CH16_2Dbytes_cov.png}}  &
		\subfloat[SanJose13\label{COV:SJ13:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{SJ13_2Dbytes_cov.png}}  &
		\subfloat[SanJose14\label{COV:SJ14:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
			{SJ14_2Dbytes_cov.png}}   	
		
	\end{tabular}
	\caption{\label{fig:cov} The percentage of Coverage errors -- elements $q$ such that  $q\notin P$ and $C_{q\mid P}\ge N\theta$ (false negatives).
%		The X axis represents the number of packets.
		}
\end{figure*}

==> analysis2.tex <==
\subsubsection{Two Dimensions}
\label{subsec:two}
Conditioned frequency is calculated differently for two dimensions, as
we use inclusion/exclusion principles and we need to show that these calculations are sound too.
We start by stating the following lemma:
\begin{lemma}
	\label{lemma:cp2d}(\cite{HHHMitzenmacher})
	In two dimensions,
	
	\[{C_{q|P}} = {f_q} - \sum\limits_{h \in G\left( {q|P} \right)} {{f_h}}  + \sum\limits_{h,h' \in G\left( {q|P} \right)} {f_{{\rm{glb}}\left( {h,h'} \right)}^{}} .\]
	\normalsize
\end{lemma}
%\begin{proof}
%	The proof appears in~\cite{HHHMitzenmacher}.
%\end{proof}
%\\
\noindent In contrast, Algorithm~\ref{alg:Skipper} estimates the conditioned frequency as:
\begin{lemma}
	\label{lemma:algCF2D}
	In two dimensions, Algorithm~\ref{alg:Skipper} calculates conditioned frequency in the following manner: \small\[\widehat {{C_{q|P}}} = \hat f_q^ +  - \sum\limits_{h \in G\left( {q|P} \right)} {\hat f_h^ - }  + \sum\limits_{h,h' \in G\left( {q|P} \right)} {\hat f_{{\rm{glb}}\left( {h,h'} \right)}^ + }  + 2{Z_{1 - \frac{\delta }{8}}}\sqrt {NV} .\]
	\normalsize
\end{lemma}
\begin{proof}
The proof follows from Algorithm~\ref{alg:Skipper}.
Line~\ref{line:cp} is responsible for the first element $\widehat{f_q^{+}}$ while Line~\ref{line:accSample} is responsible for the last element.
The rest is due to the function calcPredecessors in Algorithm~\ref{alg:randHHH2D}.
\end{proof}

%We now show that:
\begin{theorem}
	\label{thm:conservativeCP}
	$\Pr \left( {\widehat {{C_{q|P}}} \ge {C_{q|P}}} \right) \ge 1 - \delta .$
\end{theorem}
\begin{proof}
	Observe Lemma~\ref{lemma:cp2d} and notice that in deterministic~settings, as shown in~\cite{HHHMitzenmacher}, $$\widehat f_q^ +  - \sum\limits_{h \in G\left( {q|P} \right)} {\widehat f_h^ - }  + \sum\limits_{h,h' \in G\left( {q|P} \right)} \widehat f_{{\rm{glb}}\left( {h,h'} \right)}^{+}$$\normalsize
	is a conservative estimate for ${C_{q|P}}$.
	Therefore, we need to account for the randomization error and verify that with probability $1-\delta$ it is less than $2{Z_{1 - \frac{\delta }{8}}}\sqrt {NV}$.
		
	We denote by $K$ the packets that may affect $C_{q|P}$.
	Since the expression of $\widehat{C_{q|P}}$ is not monotonic, we split it into two sets: $K^{+}$ are packets that affect  $\widehat{C_{q|P}}$ positively and  $K^{-}$ affect it negatively.
	Similarly, we define $\{Y_i^K\}$ to be Poisson random variables that represent how many of the packets of $K$ are in each bin.
	
	 We do not know how many bins affect the sum, but we know for sure that there are no more than $N$ balls.
	 We define the random variable $Y^K_+$ that defines the number of packets from $K$ that fell in the corresponding bins to have a positive impact on $\widehat{C_{q|P}}$.
	 Invoking Lemma~\ref{lemma:poissonConfidence} on $Y^K_+$ yields that:
$$\Pr \left( \left| {Y_K^ +  - E\left( {Y_K^ + } \right)} \right| \ge {Z_{1-\frac{\delta }{8}}}\sqrt \frac{N}{V} \right) \le \frac{\delta }{4}.$$
	Similarly, we define $Y_{K}^-$ to be the number of packets from $K$ that fell into the corresponding buckets to create a negative impact on $\widehat{C_{q|P}}$ and Lemma~\ref{lemma:poissonConfidence} results in:
$$\Pr \left( \left| {Y_K^ -  - E\left( {{Y_K}^ - } \right)} \right| \ge {Z_{1-\frac{\delta }{8}}}\sqrt \frac{N}{V } \right) \le \frac{\delta }{4}.$$
$Y_{K}^+$ is monotonically increasing with the number of balls and $Y_{K}^-$ is monotonically decreasing with the number of balls.
We can apply Lemma~\ref{lemma:rare} and conclude that:
\small
\[\begin{array}{l}
\Pr \left( {\widehat {{C_{q|P}}} \ge {C_{q|P}}} \right) \le \\
2\Pr \left( {V\left( {Y_K^ -  + Y_K^ + } \right) \ge \left( {VE\left( {Y_K^ -  + Y_K^ + } \right) + 2{Z_{1 - \frac{\delta }{8}}}\sqrt {NV} } \right)} \right)  \\
\le 1 - 2\frac{\delta }{2} = 1 - \delta ,
\end{array}\]\normalsize completing the proof.
\end{proof}

\subsubsection{Putting It All Together}
We can now prove the coverage property for one and two dimensions.
\begin{corollary}
	\label{cor:coverage}
	If $N>\NB$ then RHHH satisfies coverage.
	That is, given a prefix $q \notin P$, where $P$ is the set of HHH returned by RHHH,  $$\Pr \left(C_{q|P}<\theta N\right) >1-\delta.$$
\end{corollary}
\begin{proof}
	The proof follows form Theorem~\ref{thm:underCP} in one dimension, or
	Theorem~\ref{thm:conservativeCP} in two, that guarantee that in both cases: $\Pr \left( C_{q|P}<\widehat{C_{q|P}}\right) > 1-\delta$.
	
	The only case where $q \notin P$ is if $\widehat{C_{q|P}}<\theta N$.
    Otherwise, Algorithm~\ref{alg:Skipper} would have added it to $P$.
	However, with probability $1-\delta$, $C_{q|P}<\widehat{C_{q|P}}$, and therefore $C_{q|P} <\theta N$ as well.
\end{proof}


\subsection{RHHH Properties Analysis}
\label{sec:RHHH-prop}
Finally, we can prove the main result of our analysis. It establishes that if the number of packets is large enough, $RHHH$ is correct.
\begin{theorem}
	\label{thm:correctness}
	If $N>\NB$, then RHHH solves {\sc {$(\delta,\epsilon, \theta)$ - Approximate Hierarchical Heavy Hitters}}.
\end{theorem}
\begin{proof}
	The theorem is proved by combining\\ Lemma~\ref{lemma:accuracy} and Corollary~\ref{cor:coverage}.
\end{proof}

Note that $\NB \triangleq \NBound$ contains the parameter $V$ in it. 
When the minimal measurement interval is known in advance, the parameter $V$ can be set to satisfy correctness at the end of the measurement. 
For short measurements, we may need to use $V=H$, while longer measurements justify using $V\gg H$ and achieve better performance. 
When considering modern line speed and emerging new transmission technologies, this speedup capability is crucial because faster lines deliver more packets in a given amount of time and thus justify a larger value of $V$ for the same measurement~interval.

For completeness, we prove the following.
\begin{theorem}
	\label{thm:O1}
	RHHH's update complexity is $O(1)$.
\end{theorem}
\begin{proof}
Observe Algorithm~\ref{alg:Skipper}.
For each update, we randomize a number between $0$ and $V-1$, which can be done in $O(1)$.
Then, if the number is smaller than $H$, we also update a Space Saving instance, which can be done in $O(1)$ as well~\cite{SpaceSavings}.
\end{proof}
Finally, we note that our space requirement is similar to that of~\cite{HHHMitzenmacher}.
\begin{theorem}
	\label{thm:space}
	The space complexity of RHHH is $O\left(\frac{H}{\varepsilon_a}\right)$ flow table entries.
\end{theorem}
\begin{proof}
RHHH utilizes $H$ separate instances of Space Saving, each using $\frac{1}{\epsilon_a}$ table entries.
There are no other space significant data~structures.
\end{proof}


==> analysisSWAMP.tex <==
\section{Analysis of SWAMP}	
\label{sec:anal}
This section is dedicated for the analysis of SWAMP.  Our analysis is partitioned into three subsections.
Section~\ref{anal:set} shows that SWAMP solves the  \SetProblem{} and the \SetMulProblem{} problems and explains the conditions where it is succinct.
It also shows that SWAMP operates in constant runtime.
Next, Section~\ref{anal:Z} shows that SWAMP solves the \CountDistinctProblem{} problem using \distinctLB{} and that \distinctMLE{} approximates its Maximum Likelihood Estimator.
Finally, Section~\ref{anal:entropy} shows that SWAMP solves \EntropyProblem{}.
%Note that SWAMP operates in constant time also when providing count distinct functionality.

%We now show that our data structure is succinct for any constant accuracy
%, we begin with the first theorem that determines the required fingerprint size.
\subsection{Analysis of per flow counting}
\label{anal:set}
We start by showing that SWAMP's runtime is constant.
\begin{theorem}
	\label{thm:runtime}
	SWAMP's runtime is \small$O(1)$\normalsize with high probability.
\end{theorem}
\begin{proof}
	\textbf{Update} - Updating the cyclic buffer requires two TinyTable operations - add and remove - both performed in constant time (with high probability) for any constant $\alpha$.
	The manipulations to $\hat{H}$ and $Z$ are also done in constant time.
	\\
	ISMEMBER - Is satisfied by TinyTable in constant time.\\
	FREQUENCY - Is satisfied by TinyTable in constant time.\\
	\textbf{\distinctLB{}} - Is satisfied by returning an integer.\\
	\textbf{\distinctMLE{}} - Is satisfied with a simple calculation.\\
	\textbf{\entropy{}} - Is satisfied by returning a floating point.
\end{proof}

Next, we prove that SWAMP solves the \SetMulProblem{} problem with regard to the function FREQUENCY (in Algorithm~\ref{alg:SWAMP}).
\begin{theorem}
	\label{thm:setmul}
SWAMP solves the \SetMulProblem{} problem.
That is, given an ID $y$, $FREQUENCY(y)$ provides an estimation $ \widehat{f^{W}_y}$ such that: 	
	$ \widehat{f^{W}_y}\ge f^{W}_y$ and
	 $\Pr \left[ {{f^{W}_y} = \widehat{f^{W}_y}} \right] \ge  1 - \varepsilon$.
\end{theorem}
\begin{proof}
	SWAMP's $CFB$ variable stores $W$ different fingerprints, each of length $L = \log_2 \left( W\epsilon^{-1} \right)$.
	For a fingerprint of size $L$, the probability that two fingerprints collide is $2^{-L}$.
    There are $W-1$ fingerprints that $h(y)$ may collide with, and $\widehat{f^{W}_y}>f^W_y$ only if it collides with one of the fingerprints in $CFB$.
%	
	Next, we use the Union Bound to~get:
	 \ifdefined\EXTENDED
	$$\Pr \left[ {f_y}^W \neq \widehat{{f_y}^W}\right] \le W \cdot {2^{ -\log_2 \left( W\epsilon^{-1}\right)}} = \varepsilon.$$
	\else
		$\Pr \left[ {f_y}^W \neq \widehat{{f_y}^W}\right] \le W \cdot {2^{ -\log_2 \left( W\epsilon^{-1}\right)}} = \varepsilon.$\\
	\fi
	Thus, given an item $y$, with probability $1-\varepsilon$, its fingerprint $\left(h(y)\right)$ is unique and TinyTable accurately measures $f^{W}_y$.
%	, that is:  	 $\Pr \left( {{f_y} = \widehat{f_y}} \right) = 1 - \varepsilon $
	Any collision of $h(y)$ with other fingerprints only increases $\widehat{f^{W}_y}$, thus $\widehat{f^{W}_y} \ge f^{W}_y$ in all cases.
	%If $H(y)$ collides with other fingerprints, then $\widehat{f_y}$ will also count the frequency of other items and then
	%$\widehat{f_y} > f_y$. We conclude that $\widehat{f_y} \ge f_y$ in all cases.
\end{proof}
Theorem~\ref{thm:setmul} shows that SWAMP solves the \SetMulProblem, which includes per flow counting and sliding Bloom filter functionalities.

Our next step is to analyze the space consumption of SWAMP.
This enables us to show that SWAMP is memory optimal to the \SetMulProblem, or more precisely, that it is succinct (according to Definition~\ref{def:succinct}).

\begin{definition}
	\label{def:succinct}
	Given an information theoretic lower bound $\mathcal B$, an algorithm is called \emph{succinct} if it uses $\mathcal B(1+o(1))$~bits.
\end{definition}
We now analyze the space consumption of SWAMP.
\begin{theorem}
	\label{thm:space}
	Given a window size $W$ and an accuracy parameter $\varepsilon$, the number of bits required by SWAMP is:
	\small
	$
	W\left(\lceil\log_2\left( W\epsilon^{-1} \right)\rceil + \left( {1 + \alpha } \right)\left( {\log_2 \epsilon^{-1} + 3} \right)\right) + o\left( { W} \right)%\mbox{\qquad \qquad bits.}
	.
	$
	\normalsize
\end{theorem}
\begin{proof}
	Our cyclic buffer ($CFB$) stores $W$ fingerprints, each of size $\lceil\log_2(W\epsilon^{-1})\rceil$, for an overall space of\\ $W\lceil\log_2\left( W\epsilon^{-1} \right)\rceil$ bits.
	Additionally, TinyTable requires: $
	\left( {1 + \alpha }  \right)W\left( {\log_2 \left( W\epsilon^{-1} \right) - \log_2 \left( W \right) + 3} \right) + o\left( W \right)$$
	$\\$
	=\left( {1 + \alpha } \right)W\left( {\log_2 \epsilon^{-1}   + 3} \right) + o\left( W \right)
	$ bits. \\Each one of the variables $curr$,  $Z$ and $\hat{H}$ require  $\log(W) = o\left(W\right)$ and thus SWAMP's memory consumption is
\ifdefined\NINEPAGES
$
W\left(\lceil\log_2\left( W\epsilon^{-1} \right)\rceil + \left( {1 + \alpha } \right)\left( {\log_2 \epsilon^{-1} + 3} \right)\right) + o\left( { W} \right).%\mbox{\qquad \qquad bits.}
$
\else	
$$
	W\left(\lceil\log_2\left( W\epsilon^{-1} \right)\rceil + \left( {1 + \alpha } \right)\left( {\log_2 \epsilon^{-1} + 3} \right)\right) + o\left( { W} \right).\qquad\qedhere%\mbox{\qquad \qquad bits.}
	$$
\fi
%	\small
%	\[
%	W\log_2\left( W\epsilon^{-1} \right) + \left( {1 + \alpha } \right)W\left( {\log_2 \left( {\frac{1}{\varepsilon }} \right) + 3} \right) + o\left( { W} \right)\] \normalsize completing the proof.
\end{proof}

\input{succinct} 

==> body.tex <==
\section{Introduction}
Network measurements are essential for a variety of network functionalities such as traffic engineering, load balancing, quality of service, caching, anomaly and intrusion detection~\cite{LBSigComm,DevoFlow,ApproximateFairness,TrafficEngeneering,IntrusionDetection2,7218487,CONGA,TinyLFU}.
A major challenge in performing and maintaining network measurements comes from rapid line rates and the large number of active flows.

Previous works suggested identifying \emph{Heavy Hitter} (HH) flows~\cite{Woodruff16} that account for a large portion of the traffic.
Indeed, approximate HH are used in many functionalities and can be captured quickly and efficiently~\cite{HashPipe,ICCCNPaper,WCSS,DIM-SUM,RAP}.
However, applications such as anomaly detection and \emph{Distributed Denial of Service} (DDoS) attack detection require more sophisticated measurements~\cite{Zhang:2004:OIH:1028788.1028802,Sekar2006}.
In such attacks, each device generates a small portion of the traffic but their combined volume is overwhelming.
HH measurement is therefore insufficient as each individual device is not a heavy hitter.
\begin{figure}[t!]
	\includegraphics[width = 0.8\columnwidth]{example-kkCD.png}
	
	\caption{A high level overview of this work. Previous algorithms' update requires $\Omega(H)$ run time, while we perform at most a single $O(1)$ update.
%		\vspace{-0.5cm}
		}
%		required conducting multiple per packet computation tasks, while our algorithm performs at most a single computation task per packet. }
	%	This speeds up the runtime, but correctness guarantees probabilistic.
	% In the deterministic model, in order to process each packet we are required to perform five different operations. In our randomized approach, we perform at most one operation for each packet, and thus the update complexity becomes constant. On the other hand, ou	r randomized approach only offers a probabilistic correctness guarantee That is, our algorithm may miss out an hierarchical heavy hitter with a small probability.
	\label{fig:contribution}
\end{figure}

\emph{Hierarchical Heavy Hitters} (HHH) account aggregates of flows that share certain IP prefixes.
The structure of IP addresses implies a prefix based hierarchy as defined more precisely below.
In the DDoS example, HHH can identify IP prefixes that are suddenly responsible for a large portion of traffic and such an anomaly may very well be a manifesting attack.
Further, HHH can be collected in one dimension, e.g., a single source IP prefix hierarchy, or in multiple dimensions, e.g., a hierarchy based on both source and destination IP~prefixes. % where the source address serves as one dimension and the destination address serves as the second.
%e.g., an edge server may need a single dimension to identify where the traffic comes from but a backbone Internet device may require two dimensions to reason about possible DDoS attacks of remote services.

Previous works~\cite{HHHMitzenmacher,CormodeHHH} suggested deterministic algorithms whose update complexity is proportional to the hierarchy's size.
These algorithms are currently too slow to cope with line speeds.
%Even with IPV4, these algorithms are too slow for current line speeds, while IPV6 further increases the size of the hierarchy and is therefore expected to further slow down current approaches.
%From an applied perspective, existing HHH algorithms are too slow to cope with modern line rates as they rely on complex algorithms that are to %too slow for modern line rates.
For example, a 100 Gbit link may deliver over 10 million packets per second, but previous HHH algorithms cannot cope with this line speed on existing hardware.
The transition to IPv6 is expected to increase hierarchies' sizes and render existing approaches even~slower.

Emerging networking trends such as \emph{Network Function Virtualization} (NFV) enable virtual deployment of network functionalities.
These are run on top of commodity servers rather than on custom made hardware, thereby improving the network's flexibility and reducing operation costs.
These trends further motivate fast software based measurement algorithms.
%This paper suggests a novel randomized HHH algorithm that operates up to 60 times faster and achieves up to x2.4 higher virtual switch throughput compared
%to previous works.

\subsection{Contributions}


First, we define a probabilistic relaxation of the HHH problem.
Second, we introduce \emph{Randomized HHH} (a.k.a. RHHH), a novel randomized algorithm that solves probabilistic HHH over single and multi dimensional hierarchical domains.
%The probabilistic guarantees of RHHH are formally analyzed and proved.
Third, we evaluate RHHH on four different real Internet traces and demonstrate a speedup of up to X62 while delivering similar accuracy and recall ratios.
Fourth, we integrate RHHH with \emph{Open vSwitch} (OVS) and demonstrate a capability of monitoring HHH at line speed, achieving a throughput of up to 13.8M packets per second.
Our algorithm also achieves X2.5 better throughput than previous approaches.
To the best of our knowledge, our work is the first to perform OVS multi dimensional HHH analysis in line speed.
%with the capability of performing HHH analysis. We demonstrate capability to

Intuitively, our RHHH algorithm operates in the following way, as illustrated in Figure~\ref{fig:contribution}:
We maintain an instance of a heavy-hitters detection algorithm for each level in the hierarchy, as is done in~\cite{HHHMitzenmacher}.
However, whenever a packet arrives, we randomly select only a single level to update using its respective instance of heavy-hitters rather than updating all levels (as was done in~\cite{HHHMitzenmacher}).
Since the update time of each individual level is $O(1)$, we obtain an $O(1)$ \emph{worst case} update time.
The main challenges that we address in this paper are in formally analyzing the accuracy of this scheme and exploring how well it works in practice with a concrete implementation.

The update time of previous approaches is $O(H)$, where $H$ is the size of the hierarchy.
An alternative idea could have been to simply sample each packet with probability $\frac{1}{H}$, and feed the sampled packets to previous solutions.
However, such a solution only provides an $O(1)$ \emph{amortized} running time.
Bounding the worst case behavior to $O(1)$ is important when the counters are updated inside the data path.
In such cases, performing an occasional very long operation could both delay the corresponding ``victim'' packet, and possibly cause buffers to overflow during the relevant long processing.
Even in off-path processing, such as in an NFV setting, occasional very long processing creates an unbalanced workload, challenging schedulers and resource allocation schemes.

%exemplify the practicality of RHHH by implementing it in a real virtual switch \emph{Open vSwitch} (OVS).
%We demonstrate a throughput improvement of X2.4 over previous algorithms in a dataplane implementation, as well as the capability to perform the measurement in an independent virtual machine.

%We evaluate RHHH in an NFV settings and achieve higher throughput compared to the alternatives.

%An example of our contribution is given in Figure~\ref{fig:contribution}, as can be observed existing deterministic algorithms are too slow and are therefore impractical for actual network components. The randomized approach suggested in this paper is up to x60 times faster than the alternatives and can process over 10 million packets per second using a single thread. This performance improvement allows our algorithms to cope with the speed of virtualized network functionalities.


%We prove traffic bounds for convergence and argue that with modern line speeds, our bounds are realistic.
%We empirically evaluate our algorithm and show a speedup of up to x30, with similar accuracy, on a variety of real Internet packet traces.
%We also show that the accuracy of our algorithm is very similar to that of its deterministic predecessors.
%Finally, we demonstrate practical capability to solve the approximate HHH problem at line rate in NFV settings and demonstrate that the improved speed of our approach translates to higher throughput of an NFV service chain that is operated on top of Open vSwitch (OVS).

% Intuitively, instead of updating the entire hierarchy

% our algorithm admits space complexity of $O\left(\frac{H}{\epsilon}\right)$ just like the state of the art~\cite{HHHMitzenmacher}, but its update time is $O(1)$ worst case. We bound the amount of traffic required for our algorithm to converge and show that given current line speeds, our bound is practical. We mathematically analyze

%We demonstrate that in practice the quality of the measurement is similar to deterministic algorithms.


%subject to constant update time, but requires a certain amount of traffic to converge. We mathematically prove that our algorithm is correct, empirically show that it is considerably faster than previous approaches and that it achieves similar accuracy. Finally, we evaluate

 %it is very similar.  demonstrate that considerably faster then the alternatives

 %Therefore, the utility of existing approaches in realistic on line network monitoring is limited as previous algorithms are simply too slow for the task.

%of these is alway proportional to the depth of the hierarchy and therefore existing solutions are simply too slow for software implementation in modern line rates. This paper suggests the first algorithm with constant update complexity for approximating HHH.

\paragraph*{Roadmap} The rest of this paper is organized as follows:
We survey related work on HHH in Section~\ref{sec:related}.
We introduce the problem and our probabilistic algorithm in Section~\ref{sec:randomized}.
For presentational reasons, we immediately move on to the performance evaluation in Section~\ref{sec:eval} followed by describing the implementation in OVS in Section~\ref{sec:ovs}.
We then prove our algorithm and analyze its formal guarantees in Section~\ref{sec:analysis}.
Finally, we conclude with a discussion in Section~\ref{sec:discussion}.

\input{table_ex}
\section{Related Work}
\label{sec:related}
%\label{sec:background}
%\subsection{HHH algorithms}

In one dimension, HHH were first defined by~\cite{Cormode2003}, which also introduced the first streaming algorithm to approximate them.
Additionally,~\cite{HHHSwitch} offered a TCAM approximate HHH algorithm for one dimension.
The HHH problem was also extended to multiple dimensions~\cite{Cormode2004,CormodeHHH,Hershberger2005,Zhang:2004:OIH:1028788.1028802,HHHMitzenmacher}.

The work of~\cite{Lin2007} introduced a single dimension algorithm that requires \small$O\left(\frac{H^2}{\epsilon}\right)$\normalsize space, where the symbol $H$ denotes the size of the hierarchy and $\epsilon$ is the allowed relative estimation error for each single flow's frequency.
Later,~\cite{Truong2009} introduced a two dimensions algorithm that requires \small $O\left(\frac{H^{3/2}}{\epsilon}\right)$\normalsize space and update time\footnote{Notice that in two dimensions, $H$ is a square of its counter-part in one dimension.}.
In~\cite{CormodeHHH}, the trie based Full Ancestry and Partial Ancestry algorithms were proposed. These use $O\left(\frac{H\log(N\epsilon)}{\epsilon}\right)$ space and requires $O\left(H\log(N\epsilon)\right)$ time per update.

The seminal work of \cite{HHHMitzenmacher}~introduced and evaluated a simple multi dimensional HHH algorithm.
Their algorithm uses a separate copy of Space Saving~\cite{SpaceSavings} for each lattice node and upon packet arrival, all lattice nodes are updated.  %with the corresponding masks.
Intuitively, the problem of finding hierarchical heavy hitters can be reduced to solving multiple non hierarchical heavy hitters problems, one for each possible query.
This algorithm provides strong error and space guarantees and its update time does not depend on the stream length.
%for two dimensions it is empirically faster than previous suggestions.
Their algorithm requires $O\left(\frac{H}{\epsilon}\right)$ space and its update time for unitary inputs is $O\left(H\right)$ while for weighted inputs it is $O\left(H \log \frac{1}{\epsilon}\right)$.

The update time of existing methods is too slow to cope with modern line speeds and the problem escalates in NFV environments that require efficient software implementations.
This limitation is both empirical and asymptotic as some settings require large hierarchies.  %and thus a complexity proportional to $H$ may be infeasible.

Our paper describes a novel algorithm that solves a probabilistic version of the hierarchical heavy hitters problem.
We argue that in practice, our solution's quality is similar to previously suggested deterministic approaches while the runtime is dramatically improved.
Formally, we improve the update time to $O(1)$, but require a minimal number of packets to provide accuracy guarantees.
We argue that this trade off is attractive for many modern networks that route a continuously increasing number of packets.




%In this paper, we suggest a randomized technique that requires $O\left(\frac{H}{\epsilon}\right)$ space, but its update time is $O(1)$.Similar to~\cite{HHHMitzenmacher}, we maintain a single Space Saving instance for each lattice node.
%We achieve dramatic speed improvement by employing a randomized update based approach where only a small number of lattice nodes are updated prior to packet arrival.
%Our approach requires a certain minimal amount of traffic in order to accurately converge.


\section{Randomized HHH (RHHH)}
\label{sec:randomized}
We start with an intuitive introductory to the field as well as preliminary definitions and notations.
Table~\ref{tbl:notations} summarizes notations used in this work.
%\subsection{Preliminaries}
\subsection{Basic terminology}
\label{sec:terminology}

We consider IP addresses to form a hierarchical domain with either bit or byte size granularity.
\emph{Fully specified} IP addresses are the lowest level of the hierarchy and can be generalized.
We use $\mathcal U$ to denote the domain of fully specified items.
For example, $181.7.20.6$ is a fully specified IP address and $181.7.20.*$ generalizes it by a single byte.
Similarly, $181.7.*$ generalizes it by two bytes and formally, a fully specified IP address is generalized by any of its prefixes.
The \emph{parent} of an item is the longest prefix that generalizes it.

In two dimensions, we consider a tuple containing source and destination IP addresses.
A fully specified item is fully specified in both dimensions.
For example,
$(\langle181.7.20.6\rangle\to \langle 208.67.222.222\rangle)$
is fully specified.
In two dimensional hierarchies, each item has two parents, e.g.,
$(\langle181.7.20.*\rangle\to \langle 208.67.222.222\rangle)$
and
$(\langle181.7.20.6\rangle\to \langle 208.67.222.*\rangle)$
are both parents to\\
$(\langle181.7.20.6\rangle\to \langle 208.67.222.222\rangle)$.

\begin{definition}[Generalization]
	For two prefixes $p,q$, we denote $p \preceq q$ if in any dimension it is either a prefix of $q$ or is equal to $q$.
	We also denote the set of elements that are generalized by $p$ with $H_p\triangleq \{e\in \mathcal U\mid e\preceq p\}$, and those generalized by a set of prefixes $P$ by $H_P\triangleq \cup_{p\in P} H_p$. If $p \preceq q$ and $p\neq q$, we denote $p\prec q$.
\end{definition}
In a single dimension, the generalization relation defines a vector going from fully generalized to fully specified.
In two dimensions, the relation defines a lattice where each item has two parents.
A byte granularity two dimensional lattice is illustrated in Table~\ref{tbl:example}.
In the table, each lattice node is generalized by all nodes that are upper or more to the left.
The most generalized node $(*,*)$ is called \emph{fully general} and the most specified node $(s1.s2.s3.s4, d1.d2.d3.d4)$ is called \emph{fully specified}.
We denote $H$ the hierarchy's size as the number of nodes in the lattice.
For example, in IPv4, byte level one dimensional hierarchies imply $H=5$ as each IP address is divided into four bytes and we also allow querying $*$.

\begin{definition}
	Given a prefix $p$ and a set of prefixes $P$,
	we define $G(p|P)$ as the set of prefixes:
	$$\left\{ {h:h \in P,h \prec p,\nexists\,h' \in P\,\,s.t.\,h \prec h' \prec p} \right\}.$$
\end{definition}
Intuitively, $G(p|P)$ are the prefixes in $P$ that are most closely generalized by $p$.
E.g., let $p=<142.14.*>$ and the set \\$P = \left\{ {<142.14.13.*>,<142.14.13.14>} \right\}$, then $G(p|P)$ only contains $<142.14.13.*>$.


We consider a stream $\mathbb{S}$, where at each step a packet of an item $e$ arrives.
Packets belong to a hierarchical domain of size $H$, and can be generalized by multiple prefixes as explained above. %in Section~\ref{sec:terminology}.
Given a fully specified item $e$, $f_e$ is the number of occurrences $e$ has in $\mathbb{S}$.
Definition~\ref{def:frequency} extends this notion to prefixes.
\begin{definition} (Frequency)
	\label{def:frequency}
	Given a prefix $p$, the frequency of $p$ is: $$f_p \triangleq \sum\nolimits_{e \in H_p} {f_e} .$$
\end{definition}

%The current number of packets in the stream is denoted $N$.


%The hierarchical heavy hitters set can be seen as a compact description of the network traffic and there are many possi

%and different algorithms are compared to one another (among other factors) by the size of their HHH set.

Our implementation utilizes Space Saving~\cite{SpaceSavings}, a popular (non hierarchical) heavy hitters algorithm, but other algorithms can also be used.
Specifically, we can use any \emph{counter algorithm} that satisfies Definition~\ref{Def:probFE} below and can also find heavy hitters, such as~\cite{frequent4,BatchDecrement,LC}.
We use Space Saving because it is believed to have an empirical edge over other algorithms~\cite{SpaceSavingIsTheBest,SpaceSavingIsTheBest2009,SpaceSavingIsTheBest2010}.

\input{notationsTable}
\normalsize

%Given a flow id, ($x$) we denote
%$B_x\triangleq \sum w_x^i .$ as the total \textbf{byte} traffic of $x$.
%Similarly, $P_x\triangleq \sum_{p_i = <x,w^i>}1$ is the total \textbf{packet} traffic of $x$.

%We denote by $\widehat{f^+_x}$ the upper estimation of $f_x$ and by $\widehat{f^{-}_x}$ the lower estimation, in our case these are the ones provided by Space Saving, in the general case these can be deduced by adding or subtracting $\epsilon \cdot N$ from $\widehat{f_x}$ as implied by definition~\ref{def:FrequencyEstimation}.
%\begin{definition}
%\label{def:FrequencyEstimation}
%An algorithm solves the
%{\sc {$(\epsilon)$ - Frequency Estimation}}: if for any set of prefixes ($x$), ESTIMATE(x) returns an estimator $\widehat{f_{x}}$ s.t:
%$$\left| {{f_{ {x} }} - \widehat {{f_{x}}}} \right| \le \varepsilon N.$$

%\end{definition}

The minimal requirements from an algorithm to be applicable to our work are defined in Definition~\ref{Def:probFE}.
This is a weak definition and most counter algorithms satisfy it with $\delta =0$.
Sketches~\cite{CountSketch,CMSketch,TinyTable} can also be applicable here, but to use them, each sketch should also maintain a list of heavy hitter items (Definition~\ref{def:HH}).
\begin{definition}
\label{Def:probFE}
An algorithm solves the {\sc {$(\epsilon, \delta)$ - Frequency Estimation}} problem if for any prefix ($x$),
it provides  $\widehat{f_{x}}$ s.t.:
$$\Pr \left[ {\left| {{f_x} - \widehat {{f_x}}} \right| \le \varepsilon N} \right] \ge 1 - \delta . $$
\end{definition}

\begin{definition}[Heavy hitter (HH)]\label{def:HH}
Given a threshold $(\theta)$, a fully specified item $(e)$ is a \textbf{heavy hitter} if its frequency $(f_e)$ is above the threshold:  $\theta \cdot N$, i.e., $f_e \ge \theta\cdot N$.
\end{definition}



%Note that this is just the definition, in practice calculating the exact conditioned frequency especially in multi dimensional domains is complicated and requires using the inclusion exclusion formula. In practice, we can only derive estimates of the conditioned frequency of prefixes, and the accuracy of these estimates will determine the size of the returned HHH set.
Our goal is to identify the hierarchical heavy hitter prefixes whose frequency is above the threshold $(\theta \cdot N)$.
However, if the frequency of a prefix exceeds the threshold then so is the frequency of all its ancestors.
For compactness, we are interested in prefixes whose frequency is above the threshold due to non HHH siblings.
This motivates the definition of  \emph{conditioned frequency} ($C_{p|P}$).
Intuitively, $C_{p|P}$ measures the \textbf{additional} traffic prefix $p$ adds to a set of previously selected HHHs ($P$), and it is defined as follows.
%
%We continue with the definition of conditioned frequency, which reflects the contribution a prefix ($p$) has to an already selected set of HHH prefixes ($P$).
\begin{definition} (Conditioned frequency)
	\label{def:cf}
	The conditioned frequency of a prefix $p$ with respect to a prefix set $P$ is: $$C_{p\mid P}\triangleq\allowbreak \sum_{e\in H_{(P\cup\{p\})} \setminus H_P} f_e.$$
\end{definition}
$C_{p\mid P}$ is derived by subtracting the frequency of fully specified items that are already generalized by items in $P$ from $p$'s frequency ($f_p$).
In two dimensions, exclusion inclusion principles are used to avoid double counting.

We now continue and describe how exact hierarchical heavy hitters (with respect to $C_{p\mid P}$) are found.
To that end, partition the hierarchy to levels as explained in Definition~\ref{Def:L}.

\begin{definition}[Hierarchy Depth]
	\label{Def:L}
	Define $L$, the \emph{depth of a hierarchy}, as follows:
    Given a fully specified element $e$, we consider a set of prefixes such that:  $e \prec p_1 \prec p_2,..\prec p_L$ where $e \neq p_1 \neq p_2 \neq ... \neq p_{L}$ and $L$ is the maximal size of that set.
	We also define the function $level(p)$ that given a prefix $p$ returns $p$'s maximal location in the chain, i.e., the maximal chain of generalizations that ends in $p$.
\end{definition}

To calculate exact heavy hitters, we go over fully specified items ($level  0$) and add their heavy hitters to the set $HHH_0$.
Using $HHH_0$, we calculate conditioned frequency for prefixes in $level 1$ and if $C_{p|{HHH_0}} \ge \theta \cdot N$ we add $p$ to $HHH_1$.
We continue this process until the last level ($L$) and the exact heavy hitters are the set $HHH_L$. Next, we define $HHH$ formally.
%This calculation is formally explained in Definition~\ref{def:HHH}.

\begin{definition}[Hierarchical HH (HHH)]
	\label{def:HHH}
	
		 The set $HHH_0$ contains the fully specified items $e$ s.t. $f_e \ge \theta\cdot N$.
		 Given a prefix $p$ from level($l$), $0\le l\le L$, we define:
		\[\begin{array}{l} HH{H_l} = 
		HH{H_{l -1}} \cup \left\{ {p:\left( {p \in level\left( l \right) \wedge {C_{p|HH{H_{l - 1}}}} \ge \theta  \cdot N} \right)} \right\} .
		\end{array}\]
	 The set of exact hierarchical heavy hitters $HHH$ is defined as the set $HHH_L$.
\end{definition}

For example, consider the case where $\theta N =100$ and assume that the following prefixes with their frequencies are the only ones above $\theta N$.
$p_1 = (<101.*>, 108)$ and $p_2 = (<101.102.*>, 102)$.
Clearly, both prefixes are heavy hitters according to Definition~\ref{def:HH}.
However, the conditioned frequency of $p1$ is $108-102  = 6$ and that of $p_2$ is 102.
Thus only $p_2$ is an HHH prefix.

Finding exact hierarchical heavy hitters requires plenty of space.
Indeed, even finding exact (non hierarchical) heavy hitters requires linear space~\cite{TCS-002}.
Such a memory requirement is prohibitively expensive and motivates finding approximate HHHs.  %Definition~\ref{def:approxHHH} of approximate HHHs.

\begin{definition}[$(\epsilon,\theta)-$approximate HHH]
\label{def:approxHHH}
An algorithm solves {\sc {$(\epsilon, \theta)$ - Approximate Hierarchical Heavy Hitters}} if after processing any stream $\mathbb{S}$ of length $N$, it returns a set of prefixes ($P$) that satisfies the following conditions:
%	We say that an algorithm solves {\sc {$(\epsilon, \delta)$ - Approximate Hierarchical Heavy Hitters}} if after processing any stream $\mathbb{S}$ of length $N$, it is able to produce a
%	set of prefixes ($Q$) that satisfies the following conditions:
	\begin{itemize}
		\item \textbf{Accuracy:} for every prefix $p\in P$,  ${\left| {{f_p} - \widehat {{f_p}}} \right| \le \varepsilon N}$.
		\item \textbf{Coverage:} for every prefix $q \notin P$:  ${{C_{q|P}} < \theta N}$.
	\end{itemize}
\end{definition}
Approximate HHH are a set of prefixes ($P$) that satisfies accuracy and coverage; there are many possible sets that satisfy both these properties.
Unlike exact HHH, we do no require that for $p \in P$, $C_{p|P} \ge \theta N$.
Unfortunately, if we add such a requirement then~\cite{Hershberger2005} proved a lower bound of $\Omega\left(\frac{1}{\theta^{d+1}}\right)$ space, where $d$ is the number of dimensions.
This is considerably more space than is used in our work ($\frac{H}{\epsilon}$) that when $\theta \propto \epsilon$ is also $\frac{H}{\theta}$.

Finally, Definition~\ref{def:deltaapproxHHH} defines the probabilistic approximate HHH problem that is solved in this paper.
\begin{definition}[$(\delta,\epsilon,\theta)-$approximate HHHs]
	\label{def:deltaapproxHHH}
	 An algorithm $\mathbb A$ solves {\sc {$(\delta,\epsilon, \theta)$ - Approximate Hierarchical Heavy Hitters}} if after processing any stream $\mathbb{S}$ of length $N$, it returns a set of prefixes $P$ that, for an arbitrary run of the algorithm, satisfies the following:
	 %such that given all runs of the algorithm and their resulting sets of prefixes $\{P\}$, when selecting an arbitrary such run and its corresponding set $P$, we have:\\
 %(which is a random variable that depends on $\mathbb A$'s randomization throughout the processing of $\mathbb S$) that satisfies the following conditions:\\
 \begin{itemize}
\item \textbf{Accuracy:} for every prefix $p\in P$, $$\Pr \left( {\left| {{f_p} - \widehat {{f_p}}} \right| \le \varepsilon N} \right) \ge 1 - \delta.$$
\item \textbf{Coverage:} given a prefix $q \notin P$,  $$\Pr \left( {{C_{q|P}} < \theta N} \right) \ge 1 - \delta .$$
\end{itemize}
%		\item 	\textbf{Coverage:} given a prefix $q$ such that $C_{q|Q}\ge\theta N$,
%			\[\Pr \left( q\in Q \right) \ge 1 - \delta .\]

\end{definition}
Notice that this is a simple probabilistic relaxation of Definition~\ref{def:approxHHH}.
Our next step is to show how it enables the development of faster algorithms.

\begin{algorithm}[h]
	%\footnotesize
	\begin{algorithmic}[1]
\Statex Initialization: $\forall d\in[L]: HH[d] =$ HH\_Alg $(\epsilon_a^{-1})$
		\Function{Update}{ $x$}
		\State $d = randomInt(0,V)$
		\If {$d<H$}
		\State Prefix $p = x\&HH[d].mask$ \Comment{Bitwise AND}
		\State $HH[d].INCREMENT(p)$
		\EndIf
		\EndFunction

		\Function{Output}{$\theta$}
		\State $P = \phi$
		\For{Level $l = |H|$ down to $0$. }
		\For{ each $p$ in level $l$}
		\State \label{line:cp}$\widehat{C_{p|P}} = \widehat{f_p}^{+} + calcPred(p,P) $
		\State \label{line:accSample}$\widehat{C_{p|P}} = \widehat{C_{p|P}}+ 2{{Z_{1 - {\delta}}}\sqrt {NV} }$
		\If {$\widehat{C_{p|P}}\ge \theta N$}
		\State $ P = P \cup \{p\}$ \Comment{$p$ is an HHH candidate}
		\State $print\left(p, \widehat{f_p}^{-}, \widehat{f_p}^{+}\right)$
		\EndIf
		\EndFor
		\EndFor
		\State\Return $P$
		\EndFunction
		
	\end{algorithmic}
\normalsize
	\caption{Randomized HHH algorithm}
	\label{alg:Skipper}
\end{algorithm}

\begin{algorithm}[h]
	%\footnotesize
	\begin{algorithmic}[1]
		\Function{calcPred}{prefix $p$, set $P$}
		\State $R = 0$
		\For{ each $h\in G(p|P)$}
		\State \label{alg:first}$R = R - \widehat{f_h}^{-}$
		\EndFor
		\State \Return $R$
		\EndFunction
	\end{algorithmic}
	\normalsize
	\caption{calcPred for one dimension }
	\label{alg:randHHH}
\end{algorithm}

\begin{algorithm}[h]
	%\footnotesize
	\begin{algorithmic}[1]
		\Function{calcPred}{prefix $p$, set $P$}
		\State $R = 0$
		\For{ each $h\in G(p|P)$}
		\State \label{alg:second}$R = R - \widehat{f_h}^{-}$
		\EndFor
		\For{ each pair $h,h'\in G(p|P)$}
		\State $q=glb(h,h')$
		\If {$\not\exists h_3 \neq h,h'\in G(p|P), q \preceq h_3$}
		\State \label{alg:third}$R = R + \widehat{f_q}^{+}$
		\EndIf
		\EndFor
		\State \Return $R$
		\EndFunction
	\end{algorithmic}
	\normalsize
	\caption{calcPred for two dimensions}
	\label{alg:randHHH2D}
\end{algorithm}

%\input{firstgraphs}
\subsection{Randomized HHH}
Our work employs the data structures of~\cite{HHHMitzenmacher}.
That is, we use a matrix of $H$ independent HH algorithms, and each node is responsible for a single prefix pattern.

\input{acc-cov.tex}
\input{graphs}
%As mentioned before, we use Space Saving~\cite{SpaceSavings} as the underlying algorithm, but other HH algorithms can be used as well.

Our solution, \emph{Randomized HHH} (RHHH), updates \textbf{at most a single} randomly selected HH instance that operates in $O(1)$.
In contrast,~\cite{HHHMitzenmacher} updates \textbf{every} HH algorithm for each packet and thus operates in $O(H)$.

Specifically, for each packet, we randomize a number between 0 and $V$ and if it is smaller than $H$, we update the corresponding HH algorithm.
Otherwise, we ignore the packet.
Clearly, $V$ is a performance parameter: when $V=H$, every packet updates one of the HH algorithms whereas when $V\gg H$, most packets are ignored.
Intuitively, each HH algorithm receives a \emph{sample} of the stream.
We need to prove that given enough traffic, hierarchical heavy hitters can still be extracted.
%Our analysis in Section~\ref{sec:analysis} formulates this intuition.

Pseudocode of RHHH is given in Algorithm~\ref{alg:Skipper}.
RHHH uses the same algorithm for both one and two dimensions.
The differences between them are manifested in the $calcPred$ method.
Pseudocode of this method is found in Algorithm~\ref{alg:randHHH} for one dimension and in Algorithm~\ref{alg:randHHH2D} for two dimensions.


%We use the following notations:
\begin{definition}
	The underlying estimation provides us with upper and lower estimates for the number of times prefix $p$ was updated ($X_p$).
    We denote: $\widehat{X^p}^{+}$ to be an upper bound for $X_p$ and $\widehat{X^p}^{-}$ to be a lower bound.
	For simplicity of notations, we define the following:\\
	$\widehat{f_p}\triangleq \widehat{X^p} V$ -- an estimator for $p$'s frequency.\\
	$\widehat{f_p^{+}}\triangleq \widehat{X^p}^{+} V$ -- an upper bound for $p$'s frequency.\\
	$\widehat{f_p^{-}}\triangleq \widehat{X^p}^{-} V$ -- a lower bound for $p$'s frequency.

\end{definition}
Note these bounds ignore the sample error that is accounted separately in the analysis.

The output method of RHHH starts with fully specified items and if their frequency is above $\theta N$, it adds them to $P$.
Then, RHHH iterates over their parent items and calculates a conservative estimation of their conditioned frequency with respect to $P$.
Conditioned frequency is calculated by an upper estimate to ($f_p^{+}$) amended by the output of the $calcPred$ method.
In a single dimension, we reduce the lower bounds of $p$'s closest predecessor HHHs.
In two dimensions, we use inclusion and exclusion principles to avoid double counting.
In addition, Algorithm~\ref{alg:randHHH2D} uses the notation of \emph{greater lower bound (glb)} that is formally defined in Definition~\ref{def:glb}.
Finally, we add a constant to the conditioned frequency to account for the sampling error.
%Once the fully specified items are done, the algorithm go over their parent items, and the variable $\Delta_p$ summarize the total frequency of their sibling heavy hitters. Prefixes that remain above $\theta N$ are reported heavy hitters. The process repeats until we reach the fully general prefix.


%and proceed gradually for fully generalized items. Since an heavy hitter prefix implies that all predecessors are also heavy hitters, we reduce repeatitions and adjust frequency estimates of heavy hitters items by reducing the frequencies of their heavy hitter siblings. This metric is called conditioned frequency and is formally defined below.

%In two dimensions, two prefixes can have common decedents, thus we need to use inclusion exclusion principles to avoid double counting. Definition~\ref{def:glb} helps us avoid double counting.

\begin{definition}
	\label{def:glb}
	Denote $glb(h,h')$ the greatest lower bound of $h$ and $h'$.
	$glb(h,h')$ is a unique common descendant of $h$ and $h'$ s.t. $\forall p : \left(q\preceq p\right)\wedge \left(p \preceq h\right)\wedge \left(p \preceq h'\right) \Rightarrow p = q.$
	When $h$ and $h'$ have no common descendants, define $glb(h,h')$ as an item with count $0$.
\end{definition}

In two dimensions, $C_{p|P}$ is first set to be the upper bound on $p$'s frequency (Line~\ref{line:cp}, Algorithm~\ref{alg:Skipper}).
Then, we remove previously selected descendant heavy hitters (Line~\ref{alg:second}, Algorithm~\ref{alg:randHHH2D}).
Finally, we add back the common descendant (Line~\ref{alg:third}, Algorithm~\ref{alg:randHHH2D})).

Note that the work of~\cite{HHHMitzenmacher} showed that their structure extends to higher dimensions, with only a slight modification to the Output method to ensure that it conservatively estimates the conditioned count of each prefix.
As we use the same general structure, their extension applies in our case as well.


==> contributiontable.tex <==
		\begin{tabular}{|c|c|c|}
	\hline 
	Problem & Estimator's Name and notation & Guarantee\tabularnewline
	\hline 
	\hline 
	\multirow{2}{*}{\SetProblem} & \multirow{2}{*}{ISMEMBER} & $\Pr(true|x\in S^W) =1$ \tabularnewline
	\cline{3-3} 
	&  & $\Pr(true|x\notin S^W) =1-\epsilon$\tabularnewline
	\hline 
	\SetMulProblem & FREQUENCY $(\widehat{f_x})$ & $\Pr\left(\widehat{f_x}\neq f_x\right) = \epsilon$\tabularnewline
	\hline 
	\multirow{2}{*}{\CountDistinctProblem} & \distinctLB{} $(Z)$ & $\Pr \left( { D - Z \ge \frac{1}{2}\varepsilon D \cdot \log \left( {\frac{2}{\delta }} \right)} \right) \le \delta.$\tabularnewline
	\cline{2-3} 
	& \distinctMLE{}$(\hat{D})$  & $\Pr \left( { \left|D - \hat{D}\right| \ge \frac{1}{2}\varepsilon D \cdot \log \left( {\frac{2}{\delta }} \right)} \right) \le \delta.$\tabularnewline
	\hline 
	\EntropyProblem & ENTROPY $(\hat{H})$ & $ \Pr \left ( H - \widehat{H} \ge \epsilon\delta^{-1} \right ) \ge 1 - \delta .$\tabularnewline
	\hline 
\end{tabular}

==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}
This work is about realizing hierarchical heavy hitters measurement in virtual network devices.
Existing HHH algorithms are too slow to cope with current improvements in network technology.
Therefore, we define a probabilistic relaxation of the problem and introduce a matching randomized algorithm called RHHH.
Our algorithm leverages the massive traffic in modern networks to perform simpler update operations.
Intuitively, the algorithm replaces the traditional approach of computing all prefixes for each incoming packets by sampling (if $V>H$) and then choosing one \emph{random} prefix to be updated.
While similar convergence guarantees can be derived for the simpler approach of updating all prefixes for each sampled packet, our solution has the clear advantage of processing elements in $O(1)$ worst case time.

We evaluated RHHH on four real Internet packet traces, consisting over 1 billion packets each and achieved a speedup of up to X62 compared to previous works.
Additionally, we showed that the solution quality of RHHH is comparable to that of previous work.
RHHH performs updates in constant time, an asymptotic improvement from previous works whose complexity is proportional to the hierarchy's size.
This is especially important in the two dimensional case as well as for IPv6 traffic that requires larger~hierarchies.

Finally, we integrated RHHH into a DPDK enabled Open vSwitch and evaluated its performance as well as the alternative algorithms.
We provided a dataplane implementation where HHH measurement is performed as part of the per packet routing tasks.
In a dataplane implementation, RHHH is capable of handling up to 13.8 Mpps, $4\%$ less than an unmodified DPDK OVS (that does not perform HHH measurement).
We showed a throughput improvement of X2.5 compared to the fastest dataplane implementations of previous~works.

Alternatively, we evaluated a distributed implementation where RHHH is realized in a virtual machine that can be deployed in the cloud and the virtual switch only sends the sampled traffic to RHHH.
Our distributed implementation can process up to 12.3 Mpps.
It is less intrusive to the switch, and offers greater flexibility in virtual machine placement.
Most importantly, our distributed implementation is capable of analyzing data from multiple network~devices.

Notice the performance improvement gap between our direct implementation -- X62, compared to the performance improvement when running over OVS -- X2.5.
In the case of the OVS experiments, we were running over a $10$Gbps link, and were bound by that line speed -- the throughput obtained by our implementation was only $4\%$ lower than the unmodified OVS baseline (that does nothing).
In contrast, previous works were clearly bounded by their computational overhead.
Thus, one can anticipate that once we deploy the OVS implementation on faster links, or in a setting that combines traffic from multiple links, the performance boost compared to previous work will be closer to the improvement we obtained in the direct~implementation.

%Unlike previous works, RHHH requires a minimal traffic volume to provide formal accuracy guarantees.
A downside of RHHH is that it requires some minimal number of packets in order to converge to the desired formal accuracy guarantees.
In practice, this is a minor limitation as busy links deliver many millions of packets every second. %s. % even before the formal accuracy guarantee is reached.
For example, in the settings reported in Section~\ref{sec:acc+cov-error}, RHHH requires up to $100$ millions packets to fully converge, yet even after as little as $8$ millions packets, the error reduces to around $1\%$.
With a modern switch that can serve $10$ million packets per second, this translates into a $10$ seconds delay for complete convergence and around $1\%$ error after $1$ second.
As line rates will continue to improve, these delays would become even shorter accordingly. The code used in this work is open sourced~\cite{RHHHCode}

\paragraph*{Acknowledgments}
We thank Ori Rottenstreich for his insightful comments and Ohad Eytan for helping with the code release.
We would also like to thank the anonymous reviewers and our shepherd, Michael Mitzenmacher, for helping us improve this work.

This work was partially funded by the Israeli Science Foundation grant \#$1505/16$ and the Technion-HPI research school.
%
Marcelo Caggiani Luizelli is supported by the research fellowship program funded by CNPq (201798/2015-8).

%We achieved x2.5 higher throughput than previous algorithms and demonstrated a capability to perform HHH measurement on OVS with minimal (>3\%) overheads.
%Alternatively, our distributed implementation has about 18\% overheads but enables the flexibility of performing the measurement in a separate virtual machine and of potentially aggregating measurements from multiple devices.













	
	


%This work demonstrates the feasibility and practicality of traffic sampling in virtualized environments. The introduction of these technologies brings us to rethink previous assumptions and we introduce a cross layer approach to network measurement where part of the solution is implemented in a virtual network device and part of it in a virtual machine.


%This work demonstrates that the development of network visualization technologies should bring us to rethink some of the key assumptions in network measurements. This paper investigate the practical usage of samples to monitor per flow byte counts, where commonly available random packet samples are unsatisfactory. We suggest a new sampling method called BUS, rigorously analyze it and derive meaningful statistical properties.  We then empirically evaluate BUS and shows that it is always more accurate than random packet samples. Moreover, in workloads where large TCP packets pose a non trivial portion of the traffic, BUS requires up to 50 times less samples ot match the accuracy of random packet samples.

%We formed a monitoring service by combining BUS with an unmodified streaming algorithms, where the streaming algorithm is used to efficiently represent BUS samples with a minimal amount of space. Surprisingly, we demonstrated that our monitoring service poses a contribution to stream processing algorithms as it operates at $O(1)$ complexity whereas the alternatives only operate at logarithmic time complexity.

%Finally, we extended a popular virtual switch (OVS) to support sampling and integrated BUS into that platform. We evaluated our implementation under typical NFV settings and found showed that the sampling overheads are reasonable and that BUS has similar overheads to random packet sampling. In our implementation, sampling yields a reasonable reduction of $\approx 9\%$ in throughput when compared to not sampling at all and an improvement of above $20\%$ when compared with sampling everything.


==> evaluation.tex <==
\newcommand{\FRHHH}{10-RHHH}
\section{Evaluation}
\label{sec:eval}


Our evaluation includes MST~\cite{HHHMitzenmacher}, the Partial and Full Ancestry~\cite{CormodeHHH} algorithms and two configurations of RHHH, one with $V=H$ (RHHH) and the other with $V=10\cdot H$ (10-RHHH).
RHHH performs a single update operation per packet while \FRHHH{} performs such an operation only for 10\% of the packets.
Thus, \FRHHH{} is considerably faster than RHHH but requires more traffic to converge.

%We considered source hierarchies in byte (1D Bytes) and bit (1D bits) granularities, as well as a source/destination byte hierarchy (2D Bytes).
%Such hierarchies were also considered by previous works~\cite{HHHMitzenmacher,CormodeHHH,HHHSwitch}.

The evaluation was performed on a single Dell 730 server running Ubuntu 16.04.01 release.
The server has 128GB of RAM and an Intel(R) Xeon(R) CPU E5-2667 v4 @ 3.20GHz processor.

Our evaluation includes four datasets, each containing a mix of 1 billion UDP/TCP and ICMP packets collected from major backbone routers in both Chicago~\cite{CAIDACH15,CAIDACH16} and San Jose~\cite{CAIDASJ13,CAIDASJ14} during the years 2014-2016.
We considered source hierarchies in byte (1D Bytes) and bit (1D Bits) granularities, as well as a source/destination byte hierarchy (2D Bytes).
Such hierarchies were also used by~\cite{HHHMitzenmacher,CormodeHHH}.
We ran each data point $5$ times and used two-sided Student's t-test to determine 95\% confidence intervals.



\subsection{Accuracy and Coverage Errors}
\label{sec:acc+cov-error}
RHHH has a small probability of both accuracy and coverage errors that are not present in previous algorithms.
Figure~\ref{fig:acc} quantifies the accuracy errors and Figure~\ref{fig:cov} quantifies the coverage errors.
As can be seen, RHHH becomes more accurate as the trace progresses.
Our theoretic bound ($\NB$ as derived in Section~\ref{sec:analysis} below) for these parameters is about 100 million packets for RHHH and about 1 billion packets for \FRHHH{}.
Indeed, these algorithms converge once they reach their theoretical bounds (see Theorem~\ref{thm:correctness}).
%For confidence ($\delta =0.001$) and sampling error, $\varepsilon_s = 0.001$, our theoretic bound ($\NB$) is about



%once these algorithms reach their theoretical bound, the error rates are indeed very small.
%\textbf{Ran: The error should be larger than $\varepsilon_s + \varepsilon_a = 0.002$}
%he error rates of RHHH are indeed very small after 100 million packets, and these of \FRHHH{} are indeed close to 0 after 1 billion packets.

% as function of the number of packets, we set $\varepsilon_s = 0.001$ and then our theoretical bound for RHHH is: $\NB  = {Z_{\left( {1 - \frac{\delta }{2}} \right)}}25 \cdot {10^6}$. We use we estimate ${Z_{\left( {1 - \frac{\delta }{2}}$ to be 4 that gives us $\delta <0.001$. That means that we need 100 million packets for RHHH to converge and 1 billion packets for \FRHHH{} to converge. As can be observed, in practice this is indeed the case.
%Figure~\ref{fig:acc} demonstrates the accuracy of our approach as a function of the stream length.
%That is, we measure how many $HHH$ items have their estimated frequency differ by more than $\varepsilon N$ from their real frequency.
%We compare two configurations of our algorithm RHHH where $V=H$ and \FRHHH{} where $V=10\cdot H$. %%% deleted since it repeats the previous subsection %%%
%As can be observed, both RHHH and \FRHHH{} become increasingly accurate as the stream becomes longer.
%This corresponds to our analysis indicating that a certain amount of traffic is required to guarantee accuracy.

\subsection{False Positives}
Approximate HHH algorithms find all the HHH prefixes but they also return non HHH prefixes.
\emph{False positives} measure the ratio non HHH prefixes pose out of the returned HHH set.
% More accurately, the returned set $P$ might be larger than the set of exact heavy hitters HHH. We refer to the number of additional prefixes as \emph{false positives}, a common metric for the quality of the algorithm.
Figure~\ref{FPR:fig:FPR} shows a comparative measurement of false positive ratios in the Chicago 16 and San Jose 14 traces. Every point was measured for $\epsilon=0.1\%$ and $\theta=1\%$.
As shown, for RHHH and \FRHHH{} the false positive ratio is reduced as the trace progresses.
Once the algorithms reach their theoretic grantees ($\NB$), the false positives are comparable to these of previous works.
In some cases, RHHH and \FRHHH{} even perform slightly better than the alternatives.


% the MST and Full Ancestry experience very low false positive ratios.  Our algorithms have somewhat higher false positive ratios, as we conservatively account for the sampling error.
%Interestingly, Partial Ancestry has similar false positive ratio to our own algorithms.

%The false positive rates for Chicago15 and SanJose13 were similar and are omitted due to lack of space.
 % has higher false positive ratios than RHHH and even \FRHHH{}.
%As mentioned above, while previous deterministic algorithms always find a set of HHH, our algorithms finds the entire set of HHH with a certain probability. Therefore, we first evaluate the coverage of our algorithms.

\subsection{Operation Speed}

Figure~\ref{fig:speed} shows a comparative evaluation of operation speed.
Figure~\ref{SJ:Byte}, Figure~\ref{SJ:bit} and Figure~\ref{SJ:2Dbyte} show the results of the San Jose 14 trace for 1D byte hierarchy ($H=5$), 1D bit hierarchy ($H=33$) and 2D byte hierarchy ($H=25$), respectively.
Similarly, Figure~\ref{CHI:byte}, Figure~\ref{CHI:bit} and Figure~\ref{CHI:2Dbyte} show results for the Chicago 16 trace on the same hierarchical domains.
Each point is computed for $250M$ long packet traces.
%The $X$ axis is the error guarantee rather than the stream length as our update speed does not depand on .
Clearly, the performance of RHHH and \FRHHH{} is relatively similar for a wide range of $\varepsilon$ values and for different data sets.
Existing works depend on $H$ and indeed run considerably slower for large $H$ values. 

Another interesting observation is that the Partial and Full Ancestry~\cite{CormodeHHH} algorithms improve when $\varepsilon$ is small.
This is because in that case there are few replacements in their trie based structure, as is directly evident by their $O(H\log(N\epsilon))$ update time, which is decreasing with $\epsilon$.
However, the effect is significantly lessened when $H$ is large.


%We also notice a performance improvement for very small $\varepsilon$ for the trie based Partial Ancestry and Full Ancestry algorithms.
%This is directly evident by their $O(H\log(N\epsilon))$ update time which is decreasing in $\epsilon$.
%nevertheless, it depends on $N$ and thus the algorithms becomes slower as the stream size increases.

%we can see that they are indeed affected by $H$.
%These algorithms perform faster for small one dimensional hierarchies (H=5) then they do for two dimensional byte granularity hierarchies (H=25) as well as one dimensional bit granularity hierarchies (H=33).

%explained by the ability of these algorithms to shorten the update process in some cases, which becomes increasingly common as their data structures grow.
%Further, in networking context, the memory requirement of such $\varepsilon$ values is often prohibitively large, especially for large hierarchies.
RHHH and \FRHHH{} achieve speedup for a wide range of $\varepsilon$ values, while \FRHHH{} is the fastest algorithm overall.
For one dimensional byte level hierarchies, the achieved speedup is up to X3.5 for RHHH and up to X10 for \FRHHH{}.
For one dimensional bit level hierarchies, the achieved speedup is up to X21 for RHHH and up to X62 for \FRHHH{}.
Finally, for 2 dimensional byte hierarchies, the achieved speedup is up to X20 for RHHH and up to X60 for \FRHHH{}.
Evaluation on Chicago15 and SanJose13 yielded similar results, which are omitted due to lack of space.
%Existing works excel on very small hierarchies such as 1 dimensional byte level hierarchies, in these cases Partial and Full Ancestry algorithms are even faster than our own RHHH for very small $\varepsilon$.
%In fact, Partial and Full Ancestry seem to be optimized for very small $\varepsilon$ values.
%\subsubsection{One dimensional byte level hierarchies}
%Figure~\ref{fig:fig:speed} shows results for 1 dimensional byte hierarchies. In these settings $H=5$, and thus the dependence of previous algorithms in $H$ does not hinder them too much. Among previous work MST is slightly faster than Partial Ancestry and Full Ancestry for large $\varepsilon$ values, and considerably slower for small values. Partial and Full Ancestry offer weaker asymptotic complexity but their design often allows early termination of the update process. Indeed, for very small $\varepsilon$ values, Partial and Full Ancestry become considerably faster than MST. It is not surprising that that RHHH and filtered RHHH are considerably faster than MST, this is by design, for a wide range of parameters RHHH is considerably faster than all previous algorithms, while filtered RHHH is faster then the rest for the entire range.

%\subsubsection{One dimensional bit level hierarchies}
%Figure~\ref{fig:speed1DBits} depicts the runtime for bit level hierarchies. In these settings it is evident that all previous work is considerably slower than our own RHHH and Filtered RHHH.  For very small $\varepsilon$ values, we notice the same improvement trend for partial and full ancestry algorithms, although their performance is still considerably slower than in the byte level case (H=5). In contrast, RHHH and Filtered RHHH operate in constant complexity and thus operate at similar speed. The achieved speedup is up to X20 for RHHH and up to X60 for Filtered RHHH.
%\subsubsection{Two dimensional byte level hierarchies}
%Figure~\ref{fig:speed2DBytes} shows the runtime for two dimensional byte level hierarchies. When considering the size of this hierarchy (H=25), it is smaller than one dimensional bit level hierarchy (H=33). Due to their constant complexity, RHHH and Filtered RHHH behave very similar to the previous cases. Previous works are considerably slower. It is interesting to notice that in this kind of hierarchies Partial Ancestry and Full Ancestry barely improve. This has to do with their early termination of updates that works more often in unidimensional hierarchies. The achieved speedup is up to X20 for RHHH and up to X60 for Filtered RHHH.


==> graphs.tex <==
%\begin{figure*}[t]
%	\captionsetup{justification=centering}
%	\begin{tabular}{ccc}
%	\subfloat[\label{FPR:SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]	{FPRGraphs/SJ14_bytes.png}} &	
%	\subfloat[SanJose14\label{FPR:SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/SJ14_bits.png}} &
%	\subfloat[SanJose14\label{FPR:SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/SJ14_2Dbytes.png}}
%	\tabularnewline
%	\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
%			{BarsLegend.png}}}		
%	\tabularnewline
%	\addtocounter{subfigure}{-1}
%	\subfloat[\label{FPR:CHI:byte}\label{FPR:`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_bytes.png}} &	
%	\subfloat[\label{FPR:CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_bits.png}} &
%	\subfloat[\label{FPR:CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
%		{FPRGraphs/CH16_2Dbytes.png}}
%	
%\end{tabular}
%	\caption{	\label{fig:acc} Accuracy error ratio -- HHH candidates whose frequency estimation error is larger than $N\epsilon$ ($\epsilon =0.001$).}		
%	%\end{figure*}	
%	%\thisfloatsetup{subfloatrowsep=qquad}
%	%\begin{figure*}[h]	
%	\captionsetup{justification=centering}
%	\begin{tabular}{cccc}
%		\multicolumn{4}{c}{\subfloat{\includegraphics[width = 7cm, height=0.6cm]
%				{ACCCOVLegend.png}}}
%		\tabularnewline
%		\addtocounter{subfigure}{-1}
%		\subfloat[Chicago15\label{COV:CH15:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{CH15_2Dbytes_cov.png}}  &
%		\subfloat[Chicago16\label{COV:CH16:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{CH16_2Dbytes_cov.png}}  &
%		\subfloat[SanJose13\label{COV:SJ13:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{SJ13_2Dbytes_cov.png}}  &
%		\subfloat[SanJose14\label{COV:SJ14:2Dbyte} - 2D Bytes]{\includegraphics[width = \fourFigWidth]
%			{SJ14_2Dbytes_cov.png}}   	
%		
%	\end{tabular}
%	\caption{\label{fig:cov} The percentage of Coverage errors -- elements $q$ such that  $q\notin P$ and $C_{q\mid P}\ge N\theta$ (false negatives).
%		%		The X axis represents the number of packets.
%	}
%\end{figure*}
%\endinput
\begin{figure*}[t]
	\begin{tabular}{ccc}
		\subfloat[\label{FPR:SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]	{FPRGraphs/SJ14_bytes.png}} &	
		\subfloat[SanJose14\label{FPR:SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/SJ14_bits.png}} &
		\subfloat[SanJose14\label{FPR:SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/SJ14_2Dbytes.png}}
		\tabularnewline
		\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
				{BarsLegend.png}}}		
		\tabularnewline
		\addtocounter{subfigure}{-1}
		\subfloat[\label{FPR:CHI:byte}\label{FPR:`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_bytes.png}} &	
		\subfloat[\label{FPR:CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_bits.png}} &
		\subfloat[\label{FPR:CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{FPRGraphs/CH16_2Dbytes.png}}
		
	\end{tabular}
	\caption{	\label{FPR:fig:FPR} False Positive Rate for different stream lengths.}
\end{figure*}



\begin{figure*}[t!]
	\begin{tabular}{ccc}
		\subfloat[\label{SJ:Byte}SanJose14 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_bytes.png}} &	
		\subfloat[SanJose14\label{SJ:bit} - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_bits.png}} &
		\subfloat[SanJose14\label{SJ:2Dbyte} - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/SJ14_2Dbytes.png}}
		\tabularnewline
		\multicolumn{3}{c}{\subfloat{\includegraphics[width = 17cm]
				{BarsLegend.png}}}		
		\tabularnewline
		\addtocounter{subfigure}{-1}
		\subfloat[\label{CHI:byte}\label{`}Chicago16 - 1D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_bytes.png}} &	
		\subfloat[\label{CHI:bit}Chicago16 - 1D Bits]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_bits.png}} &
		\subfloat[\label{CHI:2Dbyte}Chicago16 - 2D Bytes]{\includegraphics[width = \thirdFigWidth]
			{speedGraphs/CH16_2Dbytes.png}}
		
	\end{tabular}
	\caption{	\label{fig:speed} Update speed comparison for different hierarchical structures and workloads}
\end{figure*}


==> notationsTable.tex <==
\begin{table}[h]
	\centering
	

	
	\begin{tabular}{|c|l|}
		
		\hline
		Symbol & Meaning \tabularnewline
		\hline
		$\mathbb{S}$ & Stream \tabularnewline
		\hline
		$N$ & Current number of packets (in all flows)  \tabularnewline
		\hline
		$H$ & Size of Hierarchy  \tabularnewline
		\hline
		$V$ & Performance parameter, $V\ge H$  \tabularnewline
		\hline
		$S^i_x$ & Variable for the i'th appearance of a prefix $x$. 
		\tabularnewline
		\hline
		$S_{x}$ & Sampled prefixes with id $x$. 
		\tabularnewline
		\hline
		$S$ &  Sampled prefixes from all ids. 
		\tabularnewline
		
		\hline
		$\mathcal U$ & Domain of fully specified items. \tabularnewline
		\hline
		$\epsilon,\epsilon_s,\epsilon_a $ & Overall, sample, algorithm's error guarantee.  \tabularnewline
		\hline
		$\delta,\delta_s , \delta_a$ &   Overall, sample, algorithm confidence. \tabularnewline
		\hline
		$\theta$ & Threshold parameter.    \tabularnewline
		\hline

		$C_{q|P}$ & Conditioned frequency of $q$ with respect to  $P$ \tabularnewline
		\hline
		$G(q|P)$ & Subset of $P$ with the closest prefixes to q.  \tabularnewline
		\hline
		$f_q$ & Frequency of prefix q \tabularnewline
		\hline
		$\widehat{f^{+}_q},\widehat{f^{-}_q}$ & Upper,lower bound for $f_q$  \tabularnewline
		\hline
	\end{tabular}
	\caption{List of Symbols}
	\label{tbl:notations}
	
\end{table}

==> notationsTable2.tex <==
\begin{table}[h]
	\centering
	

	
	\begin{tabular}{|c|l|}
		
		\hline
		Symbol & Meaning \tabularnewline
		\hline
		$\mathbb{S}$ & Stream \tabularnewline
		\hline
		$N$ & Current number of packets (in all flows)  \tabularnewline
		\hline
		$H$ & Size of Hierarchy  \tabularnewline
		\hline
		$V$ & Performance parameter, $V\ge H$  \tabularnewline
		\hline
		$S^i_x$ & Variable for the i'th appearance of a prefix $x$. 
		\tabularnewline
		\hline
		$S_{x}$ & Sampled prefixes with id $x$. 
		\tabularnewline
		\hline
		$S$ &  Sampled prefixes from all ids. 
		\tabularnewline
		
		\hline
		$\mathcal U$ & Domain of fully specified items. \tabularnewline
		\hline
		$\epsilon,\epsilon_s,\epsilon_a $ & Overall, sample, algorithm's error guarantee.  \tabularnewline
		\hline
		$\delta,\delta_s , \delta_a$ &   Overall, sample, algorithm confidence. \tabularnewline
		\hline
		$\theta$ & Threshold parameter.    \tabularnewline
		\hline

		$C_{q|P}$ & Conditioned frequency of $q$ with respect to  $P$ \tabularnewline
		\hline
		$G(q|P)$ & Subset of $P$ with the closest prefixes to q.  \tabularnewline
		\hline
		$f_q$ & Frequency of prefix q \tabularnewline
		\hline
		$\widehat{f^{+}_q},\widehat{f^{-}_q}$ & Upper,lower bound for $f_q$  \tabularnewline
		\hline
	\end{tabular}
	\caption{List of Symbols}
	\label{tbl:notations}
	
\end{table}

==> ovsOverview.tex <==
\subsection{Open vSwitch Overview}
\label{apx:ovsOverview}

Virtual switching is a key building block in NFV environments, as it enables interconnecting multiple \emph{Virtual Network Functions} (VNFs) in service chains and enables the use of other routing technologies such as SDN. 
In practice, virtual switches rely on sophisticated optimizations to cope with the line rate.

Specifically, we target the DPDK version of OVS that enables the entire packet processing to be performed in user space. 
It mitigates overheads such as interrupts required to move from user space to kernel space. 
In addition, DPDK enables user space packet processing and provides direct access to NIC buffers without unnecessary memory copy. 
The DPDK library received significant engagement from the NFV industry~\cite{intelDpdk}.


%In kernel implementations, each arriving packet triggers an interrupt to the operating system and requires multiple copy operations (e.g., between the network interface card (NIC) and the virtual switching; or, between virtual switching and VNFs).
%Therefore, high-speed virtual switching is enabled by mitigating these overheads by various software and hardware acceleration technologies such as NetMap \cite{Rizzo-2012-Netmap} and Intel's DPDK.
%

%For these reasons, we focus our design on the DPDK-based version of OVS.
 %In this sense, DPDK-based OVS performs the entire packet processing pipeline in user space and therefore avoids the aforementioned perfomance overheads.


%
The architectural design of OVS is composed of two main components: ovs-vswitchd and ovsdb-server. 
Due to space constraints, we only describe the vswitchd component. 
The interested reader is referred to \cite{ovs-2015-nsdi} for additional information.
%
The DPDK-version of the vswitchd module implements control and data planes in user space. 
Network packets ingress the datapath (dpif or dpif-netdev) either from a physical port connected to the physical NIC or from a virtual port connected to a remote host (e.g., a VNF). 
The datapath then parses the headers and determines the set of actions to be applied (e.g., forwarding or rewrite a specific~header).


==> ovseval.tex <==
\section{Virtual Switch Integration}
\label{sec:ovs}
This section describes how we extended Open vSwitch (OVS) to include approximate HHH monitoring capabilities. For completeness, we start with a short overview of OVS and then continue with our~evaluation.
%Next, we evaluate a prototype implementation of the proposed HHH algorithms in OVS. We first provide an overview of OVS architecture. Then, we dive into how HHH are implemented in OVS and on its performance.

\input{ovsOverview}

\subsection{Open vSwitch Evaluation}
%\subsubsection{Implementation Design}

We examined two integration methods:
First, HHH measurement can be performed as part of the OVS dataplane.
That is, OVS updates each packet as part of its processing stage.
Second, HHH measurement can be performed in a separate virtual machine.
In that case, OVS forwards the relevant traffic to the virtual machine.
When RHHH operates with $V>H$, we only forward the sampled packets and thus reduce~overheads.
%\newpage

%The first uses Skipper as a dynamic sampling technique and performs the measurement in a separate virtual machine that can be placed anywhere in the cloud.
%A second option is to perform the measurement itself inside of the data plane as an integral path of the datapath.
%This alternative yields higher throughput as data is transmitted to the measurement VNF. However, this alternative creates coupling between the measurement algorithm and the virtual switch.
%These options are illustrated in Figure~\ref{fig:dut}.

%implementation where network monitoring is an integral part of the tasks performed by the datapath.

%That is, it provides the capability to dynamically adjust the sample interval, the sampled packets are then forwarded to a virtual machine that contains the measurement algorithm. This implementation offers more flexibility, and is in line with the NFV paradigm. The drawback of this implementation are the additional overheads that are imposed by switching traffic toward a separate VNF.

%It is important to note that, while our implementation deal to DPDK-accelerated datapath, they can easily be adopted to other versions.

%Second, we consider that the back box HH algorithm (in our case SSH) is running apart of OVS. This particular design is essential to understand and assess since decoupling network functionalities (in this case, the monitoring) is one of the main advantages and premises of NFV.
%
%For this implementation, we basically forward packets to the black box VNF according to the adaptive update probability. Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are just dropped.


%Our Skipper implementation extends the DPDK accelerated datapath capabilities, it is very local and only touch the dpif component, in Figure \ref{fig:ovs}. As packets are processed through the datapath, we retain easy access to the packet metadata.  Our proposed sampling implementation redefines a forwarding action as a 'branch' of the datapath. Sampled packets are actually forwarded and unsampled packets are dropped. Hence, our core implementation is simple and only requires few lines of code in dpif-netdev. Although our implementation is tailored to DPDK-accelerated user space datapath, its implementation on kernel versions is straightforward.

\subsubsection{OVS Environment Setup}
Our evaluation settings consist of two identical HP ProLiant servers with an Intel Xeon E3-1220v2 processor running at 3.1 Ghz with 8 GB RAM, an Intel 82599ES 10 Gbit/s network card and CentOS 7.2.1511 with Linux kernel 3.10.0 operating system.
The servers are directly connected through two physical interfaces.
We used Open vSwitch 2.5 with Intel DPDK 2.02, where NIC physical ports are attached using \emph{dpdk} ports.

One server is used as traffic generator while the other is used as \emph{Design Under Test (DUT)}.
Placed on the DUT, OVS receives packets on one network interface and then forwards them to the second one.
Traffic is generated using MoonGen traffic generator~\cite{MoonGen2015}, and we generate 1 billion UDP packets but preserve the source and destination IP as in the original dataset.
We also adjust the payload size to 64 bytes and reach 14.88 million packets per second (Mpps).
%MoonGen sends packets through one network interface and receives them on the other one after being processed by OVS.


%Scenario
%\subsubsection{Alternative Solutions}
%We evaluate the OVS performance considering the implementation of HHH algorithms.  We compare the performance of OVS without running any HHH algorithm (baseline) against our proposed solutions (RHHH and \FRHHH{}). We compare them to Partial Ancestry implementation.

% as part of the OVS dataplane. All implementations consider the 2D Byte version. We also compare them against the case where OVS samples the packets to a third-party VNF that implements HHH algorithms.
\begin{figure}[t]\centering
	\includegraphics[width = 0.8\columnwidth]{OVS_graphs/graph1.png}
	\caption{Throughput of dataplane implementations
		($\varepsilon = 0.001$, $\delta = 0.001$, 2D Bytes, Chicago 16).}
	\label{fig-bw1}
\end{figure}

\subsubsection{OVS Throughput Evaluation}
Figure \ref{fig-bw1} exhibits the throughput of OVS for dataplane implementations.
It includes our own \FRHHH{} (with V=10H) and RHHH (with V=H), as well as MST and Partial Ancestry.
Since we only have 10 Gbit/s links, the maximum achievable packet rate is 14.88~Mpps.

As can be seen, \FRHHH{} processes 13.8 Mpps, only 4\% lower than unmodified OVS.
RHHH achieves 10.6 Mpps, while the fastest competition is Partial Ancestry that delivers 5.6 Mpps.
Note that a 100 Gbit/s link delivering packets whose average size is 1KB only delivers $\approx$ 8.33 Mpps.
Thus, \FRHHH{} and RHHH can cope with the line speed.
%Thus, we believe that \FRHHH{} can also cope with faster interfaces.
%Alternatively, it is evident that existing works such as Partial Ancestry are too slow to cope with this line rate and only achieve up to 4 Gbit/s throughput.

%RHHH with $H=1$ achieves 8 Gbit/s throughput and thus can cope with about 11.5 million packets per second.
%This helps us establish the envelope of performance for the distributed implementation.
Next, we evaluate the throughput for different $V$ values, from $V=H=25$ (RHHH) to $V=10\cdot H =250$ (\FRHHH{}).
Figure~\ref{fig:DPI} evaluates the dataplane implementation while Figure~\ref{fig:VMI} evaluates the distributed implementation.
In both figures, performance improves for larger $V$ value. 
In the distributed implementation, this speedup means that fewer packets are forwarded to the VM whereas in the dataplane implementation, it is linked to fewer processed~packets.
\begin{figure}[t]\centering
	{\includegraphics[width = 0.8\columnwidth]{OVS_graphs/graph2b.png}}
	\caption{Dataplane implementation\label{fig:DPI}}
\end{figure}
\begin{figure}[t]\centering
	{\includegraphics[width = 0.8\columnwidth]{OVS_graphs/graph2a.png}}
%	\caption{Measured throughput in both dataplane and distributed implementations.}
	\caption{Distributed implementation\label{fig:VMI}}
%	\label{fig-bw2}
\end{figure}


%Figure~\ref{fig-bw2} shows how increasing the value of $V$ gradually increases the throughput, until the performance bottleneck becomes OVS rather than \FRHHH{}.

%The two right most bars in Figure~\ref{fig-bw2} evaluate the distributed implementation.
%When $V=H$, a distributed solution is expensive as it requires the switch to forward all traffic to the measurement VNF.
%A%lternatively, increasing $V$ to $10H$ improves the processing speed by $\approx 30\%$ to 12.3 Mpps.
Note that while the distributed implementation is somewhat slower, it enables the measurement machine to process traffic from multiple sources.
%Further, it enables a distributed deployment where multiple devices feed the same measurement VNF.
% also contains two
%also shows the overheads of only performing the initial sampling in dataplane and then forwarding $10\%$ of the traffic to a measurement VNF.
%The achieved throughput of this approach is 8.2 Gbit/s, $\approx 15\%$ less efficient than the pure dataplane implementation.
%Yet, it offers greater flexibility as the measurement VNF can be placed anywhere in the network.
%Further, it enables a distributed deployment where multiple devices feed the same measurement VNF.

%The benefit of such approach is flexibility as the measurement VNF can be placed anywhere in the network. Additionally,



%\subsubsection{Distributed implementation}

%In Figure \ref{fig-bw2}, we illustrate the impact of different filter probabilities on the overhead of \FRHHH{} method. Observe that as we increase the probability to update HHH, the throughput overhead increases (up to 25\%) since more packets update the HHH data structures. Observe that there is a tradeoff between the error and the achieved performance.
%
%Additionally, we also compare \FRHHH{} to the scenario which packets are sampled to a monitoring VNF. In this particular case, we assume that the VNF has an implementation of HHH. Then, OVS is required to forward a percentage of packets to that VNF. As OVS does not support natively sampling packets in the dataplane, we implement a packet uniform sampling method in the dataplane so as OVS also forwards packets to a virtual port (attached to the VNF). Observe, in Figure \ref{fig-bw2}, that considering a probability of 10\% on sampling the packets, higher penalties are obtained than doing it for 30\% of the packets in the dataplane.


%Figure \ref{fig-bw} shows the average end-to-end throughput on the SanJose14 trace for our two designs. Similar results were obtained when running different network traces.
%As shown, measuring the data inside the data plane is efficient and reduces the throughput by only $3\%$.
%When the measurement takes place in a dedicated VNF, Skipper increases the OVS throughput by about $25\%$.
%When the measurement is done as a part of the datapath its overheads are almost negligible and the throughput impact is less than $3\%$. The reason for that is that less traffic is routed. Alternatively, when Skipper is implemented as a VNF, the measurement reduces throughput by $13\%$, when compared to not performing measurement. Since sketches and counter based algorithms process all packets in the stream, implementing them as VNFs has higher overheads, and degrades performance by more than $30\%$.


%We clearly observe the existence of a tradeoff between flexibility and performance between the two proposed designs. Running the monitoring HH algorithm outside OVS (in a VNF) introduces higher flexibility in the implementations of new HH strategies. In turn, compiling HH algorithm as part of the OVS datapath reduce the burden of forwarding packets to a VNF.
%




==> succinct.tex <==
The work of~\cite{Naor2013} implies a lower bound for the \SetProblem{} problem of \ifdefined\EXTENDED
$$\mathcal B\triangleq W\left(\log_2 \epsilon^{-1} + \max \left( {\log_2 \log_2 \epsilon^{-1},\log_2 \left( W \right)} \right)\right)$$
\else
\\$\mathcal B\triangleq W\left(\log_2 \epsilon^{-1} + \max \left( {\log_2 \log_2 \epsilon^{-1},\log_2 \left( W \right)} \right)\right)$
\fi bits.
This lower bound also applies to our case, as SWAMP solves the \SetMulProblem{} and the \SetProblem{} by returning whether or not $\widehat{{f_y}^W}>0$.

\begin{corollary}\label{cor:bf}
SWAMP solves the \SetProblem{} problem.
\end{corollary}

%because all items that appeared in the window are estimated with positive frequency, and the chance for false positive is $\varepsilon$.
We now show that SWAMP is succinct for $\epsilon=W^{-o(1)}$.
\begin{theorem}
Let $\epsilon=W^{-o(1)}$. Then SWAMP is succinct for the \SetProblem{} and \SetMulProblem{} problems.
\end{theorem}
\begin{proof}
	Theorem~\ref{thm:space} shows that the required space~is:
\ifdefined\EXTENDED
{\footnotesize
		\begin{multline*}
		S \le W\log_2 W + W(2 + \alpha) \log_2 \epsilon^{-1} +4W + 3W\alpha
		+o(W)=\\
		W\log_2 W\cdot\left(1 + \frac{1}{\log_2 W} \left[(2 + \alpha) \log_2 \epsilon^{-1}+4+3\alpha + o(1)\right] \right)
		=  W\log_2 W\cdot\left(1 + (2 + \alpha)\frac{ \log_2 \epsilon^{-1}}{\log_2 W}  + o(1)\right).
	\end{multline*}}
\else
{\footnotesize
	$
	S \le W\log_2 W + W(2 + \alpha) \log_2 \epsilon^{-1} +4W + 3W\alpha
	+o(W)=\\
	W\log_2 W\cdot\left(1 + \frac{1}{\log_2 W} \left[(2 + \alpha) \log_2 \epsilon^{-1}+4+3\alpha + o(1)\right] \right)\\
	=  W\log_2 W\cdot\left(1 + (2 + \alpha)\frac{ \log_2 \epsilon^{-1}}{\log_2 W}  + o(1)\right).
	$}
\fi
We show that this implies succinctness according to Definition~\ref{def:succinct}.
Under our assumption that $\epsilon=W^{-o(1)}$, we get that:
$\log_2\epsilon^{-1} = \log_2(W^{o(1)}) = o(\log_2 W)$, hence SWAMP uses $W\log_2 W(1+o(1))=\mathcal{B}(1+o(1))$ bits and is~succinct.
\qedhere
% For a constant $\varepsilon$, Window Counting requires: $(1+o(1))W \log_2\left(W\right)$ bits. \textbf{Ran: can you finish this}	
\end{proof}

\subsection{Analysis of count distinct functionality}
\label{anal:Z}
We now move to analyze SWAMP's count distinct functionality.
Recall that SWAMP has two estimators; the one sided \distinctLB{} and the more accurate \distinctMLE{}.
Also, recall that $Z$ monitors the number of distinct fingerprints and that $D$ is the real number of distinct flows (on the window).

\subsubsection{Analysis of \distinctLB{}}
We now present an analysis for \distinctLB{}, showing that it solves the \CountDistinctProblem{} problem.


\begin{theorem}
	\label{thm:Z}
	$Z\le D$ and $\mathbb{E}(Z)\ge D\cdot (1-\frac{\varepsilon}{2})$.
\end{theorem}
\begin{proof}
	Clearly, $Z \le D$ always, since any two identical IDs map to the same fingerprint.
	Next, for any $0 \le i \le 2^L-1$, denote by $Z_i$ the indicator random variable, indicating whether there is some item in the window whose fingerprint is $i$.
    Then $Z = \sum_{i=0}^{2^L-1} Z_i$, hence $\mathbb{E}(Z) = \sum_{i=0}^{2^L-1} \mathbb{E}(Z_i)$.
    However
    \ifdefined\EXTENDED
    	, for any $i$,
    \fi
    \ifdefined\EXTENDED
    $$ \mathbb{E}(Z_i) = \Pr(Z_i = 1) = 1 - \left( 1 - 2^{-L} \right)^D .$$
    \else
        \small$ \mathbb{E}(Z_i) = \Pr(Z_i = 1) = 1 - \left( 1 - 2^{-L} \right)^D. $\normalsize
    \fi 
    The probability that a fingerprint is exactly $i$ is $2^{-L}$, thus:
	\begin{equation} \label{eq:DISTINCT expectation}
	\mathbb{E}(Z) = 2^L \cdot \left( 1 - \left( 1 - 2^{-L} \right)^D \right).
	\end{equation}
	Since $ 0 < 2^{-L} \le 1 $, we have:\\
	$ \left( 1 - 2^{-L} \right)^D < 1 - D \cdot 2^{-L} + {D \choose 2} \cdot 2^{-2L} $
	which, in turn, implies	$ \mathbb{E}(Z) > D - {D \choose 2} \cdot 2^{-L} $.
	Finally, we note that $2^{-L} = \frac{\varepsilon}{W}$ and that $ D \le W $.
    Hence, \small	$ \mathbb{E}(Z) > D - \frac{D(D-1)\varepsilon}{2W} > D \cdot \left( 1 - \frac{\varepsilon}{2} \right).\qedhere$\normalsize
\end{proof}

Our next step is a probabilistic bound on the error of $Z$ ($X = D-Z$).
This is required for Theorem~\ref{thm:epsDeltaDistinctLB}, which is the main result and shows that $Z$ provides an $\epsilon,\delta$ approximation for the distinct elements problem.

We model the problem as a balls and bins problem where $D$ balls are placed into $2^L = \frac{W}{\varepsilon}$ bins. The variable $X$ is the number of bins with at least $2$ balls.

For any $0\le i \le 2^L-1$, denote by $X_i$ the random variable denoting the number of balls in the $i$-th bin. Note that the variables $X_i$ are dependent of each other and are difficult to reason about directly. Luckily, $X$ is monotonically increasing and we can use a Poisson approximation.
To do so, we denote by $Y_i\sim Poisson \left( \frac{D}{2^L} \right) $ the corresponding independent Poisson variables and by $Y$ the Poisson approximation of $X$, that is $Y$ is the sum of $Y_i's$ with value 2 or more.

Our goal is to apply Lemma~\ref{lemma:rare}, which links the Poisson approximation to the exact case. In our case, it allows us to derive insight about $X$ by analyzing $Y$.

\begin{lemma}[Corollary 5.11, page 103 of~\cite{Mitzenmacher:2005:PCR:1076315}]
	\label{lemma:rare}
	Let $\mathcal{E}$ be an event whose probability is either monotonically increasing or decreasing with the number of balls. If $\mathcal{E}$ has probability $p$ in the Poisson case then $\mathcal{E}$ has probability at most $2p$ in the exact case.
	Here $\mathcal{E}$ is an event depending on $X_0,\ldots ,X_{2^L-1}$ (in the exact case), and the probability of the event in the Poisson case is obtained by computing $\mathcal{E}$ using $Y_0, \ldots ,Y_{2^L-1}$.
\end{lemma}

That is, we need to bound the probability $\Pr(X_i \ge 2)$ and to do so we define a random variable $Y$ and bound: $\Pr(Y_i \ge 2)$ which can be at most $2\cdot \Pr(X_i\ge 2)$.

We may now denote by $\tilde{Y}_i = Y_i \ge 2$ the indicator variables, indicating whether $Y_i$ has value at least 2. By definition:\\ $ Y = \sum_{i=0}^{2^L-1} \tilde{Y}_i $.
It follows that:
\ifdefined\EXTENDED
$$ \mathbb{E}(Y) = \sum_{i=0}^{2^L-1} \mathbb{E}(\tilde{Y}_i) = 2^L \cdot \Pr(Y_i \ge 2) .$$
\else
$\\ \mathbb{E}(Y) = \sum_{i=0}^{2^L-1} \mathbb{E}(\tilde{Y}_i) = 2^L \cdot \Pr(Y_i \ge 2) .$\\
\fi
$Y_i \sim Poission \left( \frac{D}{2^L} \right) $, hence:
\ifdefined\EXTENDED
$$ \Pr(Y_i \ge 2) = 1 - \Pr(Y_i = 0) - \Pr(Y_i = 1)$$$$ = 1 - e^{-\frac{D}{2^L}} \cdot \left( 1 + \frac{D}{2^{L+1}} \right) ,$$
\else
\\$ \Pr(Y_i \ge 2) = 1 - \Pr(Y_i = 0) - \Pr(Y_i = 1)$\\$ = 1 - e^{-\frac{D}{2^L}} \cdot \left( 1 + \frac{D}{2^{L+1}} \right) ,$
\fi
and thus:\\
$ \mathbb{E}(Y) = 2^L \cdot \left( 1 - e^{-\frac{D}{2^L}}  \cdot \left( 1 + \frac{D}{2^L} \right) \right) .$\\
Since $ e^{-x} \cdot (1 + x) > 1 - \frac{x^2}{2} $ for $ 0 < x \le 1$, we get
\ifdefined\EXTENDED
$$ \mathbb{E}(Y) < 2^L \cdot \left( 1 - \left( 1 - \frac{D^2}{2^{2L+1}} \right) \right) = \frac{D^2}{2^{L+1}} .$$
\else
\\$ \mathbb{E}(Y) < 2^L \cdot \left( 1 - \left( 1 - \frac{D^2}{2^{2L+1}} \right) \right) = \frac{D^2}{2^{L+1}} .$\\
\fi
Recall that $2^L = W\varepsilon^{-1}$ and $D \le W$ and thus
$ \mathbb{E}(Y) < \frac{D \cdot \varepsilon}{2} .$

Note also that the $\{\tilde{Y}_i\}$ are independent, since the $\{Y_i\}$ are independent, and as they are indicator (Bernoulli) variables, in particular they are Poisson trials.
Therefore, we may use a Chernoff bound on $Y$ as it is the sum of independent Poisson trials.
We use the following Chernoff bound to continue:
\begin{lemma}[Theorem 4.4, page 64 of~\cite{Mitzenmacher:2005:PCR:1076315}]
	\label{lemma:Chernoff}
	Let $X_1,...,X_n$ be independent Poisson trials such that: $\Pr(X_i) = p_i$, and let $X = \sum_{i=1}^{n} X_i$, then for $R\ge 6\mathbb{E}(X)$, $\Pr\left(X\ge R\right)\le 2^{-R}$.
\end{lemma}

Lemma~\ref{lemma:Chernoff} allows us to approach Theorem~\ref{thm:epsDeltaDistinctLB}, which is the main result for \distinctLB{} and shows that it provides an $\epsilon,\delta$ approximation of $D$, which we can then use in Corollary~\ref{cor:epsDeltaDistinct} to show that it solves the count distinct problem.

\begin{theorem}
	\label{thm:epsDeltaDistinctLB}
	
	Let \scriptsize$\delta \le \frac{1}{128}$\normalsize. Then:
	\ifdefined\EXTENDED	
	$$\Pr \left( { D - Z \ge \frac{1}{2}\varepsilon D \cdot \log \left( {\frac{2}{\delta }} \right)} \right) \le \delta.$$
	\else
	\scriptsize
	$\Pr \left( { D - Z \ge \frac{1}{2}\varepsilon D \cdot \log \left( {\frac{2}{\delta }} \right)} \right) \le \delta.$
	\fi
	
\end{theorem}
\begin{proof}
	For $\delta\le \frac{1}{128}$, $\log\left(\frac{2}{\delta}\right)\ge 6$ and thus, as\\
	$ \log_2\left(\frac{2}{\delta}\right) \cdot \frac{1}{2} \varepsilon D \ge 6 \mathbb{E}(Y) $ we can use Lemma~\ref{lemma:Chernoff} to get that:
	\small
	\ifdefined\EXTENDED
	\[\Pr \left( {Y \ge \frac{1}{2}\varepsilon D \cdot \log_2 \left( {\frac{2}{\delta }} \right)} \right) \le {2^{ - \left( {\varepsilon D} \right)\log_2 \left( {\frac{2}{\delta }} \right)}} \le {2^{ - \log_2 \left( {\frac{2}{\delta }} \right)}} \le \frac{\delta }{2}.\]
	\else
		$\Pr \left( {Y \ge \frac{1}{2}\varepsilon D \cdot \log_2 \left( {\frac{2}{\delta }} \right)} \right) \le {2^{ - \left( {\varepsilon D} \right)\log_2 \left( {\frac{2}{\delta }} \right)}} \le {2^{ - \log_2 \left( {\frac{2}{\delta }} \right)}} \le \frac{\delta }{2}.$
	\fi
	\normalsize
	
	As $X$ monotonically increases with $D$, we use Lemma~\ref{lemma:rare} to conclude that
	$\Pr \left( {X \ge \frac{1}{2}\varepsilon D \cdot \log_2 \left( {\frac{2}{\delta }} \right)} \right) \le \delta.~\qedhere$
\end{proof}
The following readily follows, as claimed.
\begin{corollary}
    \label{cor:epsDeltaDistinct}
    \distinctLB{} solves the\\ \CountDistinctProblem{} problem,
    for $\varepsilon_D = \frac{1}{2} \varepsilon \cdot \log_2 \left( {\frac{2}{\delta }} \right)$, and any $\delta \le \frac{1}{128}$.
    That is, for such $\delta$ we get:
    $ \Pr \left ( Z \ge (1 - \varepsilon_D ) \cdot D \right ) \ge 1 - \delta .$
\end{corollary}

\subsubsection{Analysis of \distinctMLE{}}
%{Analysis of Maximum Likelihood Estimator for distinct items (\distinctMLE{})}
\ifdefined\NINEPAGES
We state the confidence interval results derived for the MLE estimator. As the proof is highly technical it is differed to the full version~\cite{full-version}.
\begin{theorem} \label{thm:prob margin}
	Let $\delta \le \frac{1}{128} $ and denote $\varepsilon_D = \frac{1}{2} \varepsilon \cdot \log_2 \left(\frac{2}{\delta} \right)$. Then
	$ \Pr \left( \hat{D} \le D \cdot (1 - \varepsilon_D) \right) \le \delta .$
\end{theorem}
\else
We now provide an analysis of the \distinctMLE{} estimation method, which is more accurate but offers two sided error.
%Namely, we use the estimator $\hat{D} \triangleq \frac{\ln \left( 1 - \frac{Z}{2^L} \right)}{\ln \left(1 - \frac{1}{2^L} \right)}$.
Our goal is to derive confidence intervals around \distinctMLE{} and for this we require a better analysis of $Z$, which is provided by Lemma~\ref{lem:DISTINCT expectation precise}.
\begin{lemma}
	\label{lem:DISTINCT expectation precise}
	\begin{equation}
	D - {D \choose 2} \cdot 2^{-L} \le \mathbb{E}(Z) \le  D - {D \choose 2} \cdot 2^{-L} + {D \choose 3} \cdot 2^{-2L}.
	\end{equation}
\end{lemma}
\begin{proof}
	This follows simply from~\ref{eq:DISTINCT expectation} by expanding the binomial.
\end{proof}
We also need to analyze the second moment of $Z$.
Lemma~\ref{lem:DISTINCT second moment} does just that.
\begin{lemma}
	\label{lem:DISTINCT second moment}
	\begin{align*}
	\mathbb{E}(Z^2) = 2^{2L} - \left ( 2^{2L+1} - 2^L \right) \left ( 1 - \frac{1}{2^L} \right)^D 
	+ \left ( 2^{2L} - 2^L \right) \left ( 1 - \frac{1}{2^{L-1}} \right)^D.
	\end{align*}
\end{lemma}
\begin{proof}
	As in Theorem~\ref{thm:Z}, we write $Z$ as a sum of indicator variables $Z = \sum_{i=0}^{2^L-1} Z_i$. Then
	$$ Z^2 = \sum_{i=0}^{2^L-1} Z_i^2 + \sum_{i\ne j} Z_i Z_j. $$
	By linearity of the expectation, it implies
	\begin{equation} \label{eq:Z variance}
	\mathbb{E}(Z^2) = \sum_{i=0}^{2^L-1} \mathbb{E}(Z_i^2) + \sum_{i\ne j} \mathbb{E}(Z_i Z_j).
	\end{equation}
	We note that for any $i \ne j$,  $ (1-Z_i)(1-Z_j) $ is also an indicator variable, attaining the value $1$ with probability $ \left ( 1 - \frac{2}{2^L} \right)^D $.
	Therefore, for any $i \ne j $, we have by linearity of the expectation, that
	\begin{align*}
	\left ( 1 - \frac{2}{2^L} \right)^D =  \mathbb{E}(1 - Z_i)(1-Z_j) = 1 - \mathbb{E}(Z_i) - \mathbb{E}(Z_j) + \mathbb{E}(Z_i Z_j).
	\end{align*}
	Since $ \mathbb{E}Z_i = 1 - \left ( 1 - \frac{1}{2^L} \right)^D $, it follows that
	\begin{align*}
	\mathbb{E}(Z_i Z_j) = \left ( 1 - \frac{2}{2^L} \right)^D + 2 \cdot \left (  1 - \left ( 1 - \frac{1}{2^L} \right)^D \right) - 1 
		= 1 +  \left ( 1 - \frac{2}{2^L} \right)^D - 2  \left ( 1 - \frac{1}{2^L} \right)^D.
	\end{align*}
	Plugging it back in Equation~\ref{eq:Z variance}, and using $Z_i^2 = Z_i$, we obtain
	\begin{align*}
	 \mathbb{E}(Z^2) = 2^L \cdot \left (  1 - \left ( 1 - \frac{1}{2^L} \right)^D \right)
		+ 2^L (2^L - 1) \left (   1 +  \left ( 1 - \frac{2}{2^L} \right)^D - 2  \left ( 1 - \frac{1}{2^L} \right)^D \right).
	\end{align*}
	Finally, expanding and rearranging we obtain the claim of this lemma.
\end{proof}

As our interest lies in the confidence intervals, we shall only need an approximation, described in the following simple corollary

\begin{corollary}
	\label{cor:DISTINCT second moment approx}
	$ D^2 - \frac{4 \cdot D^3}{3 \cdot 2^L} < \mathbb{E}(Z^2) < D^2 + \frac{D^3}{3 \cdot 2^L}$.
\end{corollary}
\begin{proof}
	First, note that binomial expansion yields
	$$ 1 - \frac{D}{2^L} + \frac{{D \choose 2}}{2^{2L}} - \frac{{D \choose 3}}{2^{3L}} \le \left ( 1 - \frac{1}{2^L} \right)^D \le 1 - \frac{D}{2^L} + \frac{{D \choose 2}}{2^{2L}}.$$
	Plugging it back into Lemma~\ref{lem:DISTINCT second moment}, and expanding we get on the one hand
	\begin{multline*}
	\mathbb{E}(Z^2) > 2^{2L} - (2^{2L+1} - 2^L) \left ( 1 - \frac{D}{2^L} + \frac{ {D \choose 2} }{2^{2L}} \right)  
	+ (2^{2L} - 2^L) \left( 1 - \frac{D}{2^{L-1}} + \frac{ {D \choose 2}}{2^{2L-2}} - \frac{{D \choose 3}}{2^{3L-3}} \right) = \\
	= D + 2 \cdot {D \choose 2} - 2^{-L} \cdot \left( \frac{3D(D-1)}{2} + \frac{8D(D-1)(D-2)}{6} \right)
	= D^2 - \frac{D(D-1)(8D-7)}{6 \cdot 2^L},
	\end{multline*}
	which yields the lower bound.
	On the other hand, we have
	\begin{multline*}
	\mathbb{E}(Z^2) < 2^{2L} - (2^{2L+1} - 2^L) \left ( 1 - \frac{D}{2^L} + \frac{ {D \choose 2} }{2^{2L}} - \frac{{D \choose 3}}{2^{3L-3}} \right) 
	+ (2^{2L} - 2^L) \left( 1 - \frac{D}{2^{L-1}} + \frac{ {D \choose 2}}{2^{2L-2}}  \right) = \\
	= D + 2 \cdot {D \choose 2} + 2^{-L} \cdot \left(- \frac{3D(D-1)}{2} + \frac{D(D-1)(D-2)}{3} \right) 
	= D^2 + \frac{D(D-1)(2D-13)}{6 \cdot 2^L},
	\end{multline*}
	which yields the upper bound.
\ifdefined\EXTENDED	
	Thus, we have established the corollary.
\fi	
\end{proof}

Using Corollary~\ref{cor:DISTINCT second moment approx} and Lemma~\ref{lem:DISTINCT expectation precise} we can finally get an estimate for $\mathbb{E}(\hat{D})$, as described in the following theorem. This shows that $\hat{D}$ is unbiased up to an $O(D\epsilon^2)$ additive factor.

\begin{theorem}
	\label{thm:DISTINCT2 expectation}
\small
	\begin{equation}
	- D \cdot \varepsilon^2 \cdot \left( \frac{2}{3} + \frac{\varepsilon}{2W^3} \right)  < \mathbb{E}(\hat{D}) -D < D \cdot \varepsilon^2 \cdot \left(2 + \frac{1}{3(1-\varepsilon)^3} \right).
	\end{equation}
	\normalsize
\end{theorem}
\begin{proof}
	We first note that for $x \in [0,1)$ one has
	\begin{equation} \label{eq:ln approx}
	x + \frac{x^2}{2} \le -\ln (1-x) \le x + \frac{x^2}{2} +\frac{x^3}{3(1-x)^3}.
	\end{equation}
	Therefore, we have
	$$  \frac{Z}{2^L} + \frac{Z^2}{2^{2L+1}} \le - \ln \left( 1 - \frac{Z}{2^L} \right) \le \frac{Z}{2^L} + \frac{Z^2}{2^{2L+1}} + \frac{Z^3}{3 \cdot (2^L-Z)^3} .$$
	Since always $Z \le D$, and $\frac{D}{2^L} \le \frac{W}{2^L} = \varepsilon$, we can take expectation and obtain, by linearity and monotonicity of the expectation, that
	\begin{align} \label{eq:ineq expectation approx}
	\frac{\mathbb{E}(Z)}{2^L} + \frac{\mathbb{E}(Z^2)}{2^{2L+1}} \le \mathbb{E} \left( - \ln \left( 1 - \frac{Z}{2^L} \right) \right) 
 	\le \frac{\mathbb{E}(Z)}{2^L} + \frac{\mathbb{E}(Z^2)}{2^{2L+1}} + \frac{D^3}{3 \cdot (2^L-D)^3}.
	\end{align}
	We can now substitute Lemma~\ref{lem:DISTINCT expectation precise} and Corollary~\ref{cor:DISTINCT second moment approx} to obtain
	\begin{multline*}
	-\mathbb{E} \left( \ln \left( 1 - \frac{Z}{2^L} \right) \right) \le \frac{D}{2^L} + \frac{D}{2^{2L+1}} + \frac{D^3}{6 \cdot 2^{3L}} 
 	+ \frac{{D \choose 3}}{2^{3L}} + \frac{D^3}{3 \cdot (2^L-D)^3} \\\le \frac{D}{2^L} + \frac{D}{2^{2L+1}}
	+ D \cdot \left( \frac{2W^2}{2^{3L}} + \frac{W^2}{3(1-\varepsilon)^3 \cdot 2^{3L}} \right).
	\end{multline*}
	Recalling~\ref{eq:ln approx} we see also that
	$ -\ln \left( 1 - \frac{1}{2^L} \right) \ge \frac{1}{2^L} + \frac{1}{2^{2L+1}} $.
	Combining both inequalities, we get
	\begin{align*}
	\mathbb{E}(\hat{D}) \le D + D \cdot \left( \frac{2W^2}{2^{2L}+2^{L-1}} + \frac{W^2}{3(1-\varepsilon)^3 \cdot (2^{2L} + 2^{L-1})} \right) \le   D + D \cdot \left( \frac{2W^2}{2^{2L}} + \frac{W^2}{3(1-\varepsilon)^3 \cdot 2^{2L}} \right).
	\end{align*}
	Since $ 2^L = W\varepsilon^{-1} $, this gives us the upper bound.
	On the other hand, substituting Lemma~\ref{lem:DISTINCT expectation precise} and Corollary~\ref{cor:DISTINCT second moment approx} in the left inequality given in~\eqref{eq:ineq expectation approx} we have also
	$$ -\mathbb{E} \left( \ln \left( 1 - \frac{Z}{2^L} \right) \right) \ge \frac{D}{2^L} + \frac{D}{2^{2L+1}} - \frac{4D^3}{6 \cdot 2^{3L}} .$$
	From~\eqref{eq:ln approx} we see also that
	$ -\ln \left( 1 - \frac{1}{2^L} \right) \le \frac{1}{2^L} + \frac{1}{2^{2L+1}} + \frac{1}{3\cdot (2^L-1)^3}. $
	Combining both inequalities, we get
	\begin{align*}
	\mathbb{E}(\hat{D}) \ge D - \frac{4D^3}{6\cdot (2^{2L} + 2^{L-1} + 3)} - \frac{8D}{3\cdot 2^{3L}} 
	\ge D - D \cdot \left( \frac{2D^2}{3\cdot 2^{2L}} + \frac{8}{3\cdot 2^{3L}} \right).
	\end{align*}
	Since $ D \le W $ and $2^L = W\varepsilon^{-1}$, this yields the lower bound, as claimed.
\end{proof}

Next, we bound the error probability. This is done in the following theorem.
\begin{theorem} \label{thm:prob margin}
	Let $\delta \le \frac{1}{128} $ and denote $\varepsilon_D = \frac{1}{2} \varepsilon \cdot \log_2 \left(\frac{2}{\delta} \right)$. Then
	$$ \Pr \left( \hat{D} \le D \cdot (1 - \varepsilon_D) \right) \le \delta .$$
\end{theorem}
\begin{proof}
We first note that
$$ \Pr \left( \frac{\ln \left( 1 - \frac{Z}{2^L} \right)}{\ln \left( 1 - \frac{1}{2^L} \right)} \le a \right) = \Pr \left( Z \le 2^L \left( 1 - \left( 1 - \frac{1}{2^L} \right)^a \right) \right) .$$
Now, using Corollary~\ref{cor:epsDeltaDistinct}, and the fact that
$$  2^L \left( 1 - \left( 1 - \frac{1}{2^L} \right)^a \right) \le a,  $$
the result immediately follows.
\end{proof}

Theorem~\ref{thm:prob margin} shows the soundness of the \distinctMLE{} estimator by proving that it is at least as accurate as the \distinctLB{} estimator.

\fi
% This might give better bounds in the future
%To do so, we quantify the convergence to the normal distribution.
%We use a technique due to Harris and Park (see \cite{Harris and Park}), of estimating the factorial cumulants.
%This was originally used to show that $Z$ converges to a normal distribution, so here we present a more refined analysis.
%We begin by writing down explicitly the distribution of $Z$. For any $ 0\le z \le 2^L$ we have by the inclusion-exclusion principle:
%$$ \Pr(Z = z) = {2^L \choose z} \sum_{i=0}^{z-1} (-1)^{i} {z \choose i} \left( \frac{z-i}{2^L} \right)^D  $$
%Denote $X = 2^L - Z$ the random variable representing the number of unused fingerprints.
%Denote, for any $r \ge 0$,  by
%$$ \mu_{(r)}(X) = \mathbb{E}(X^{(r)}) = \mathbb{E}(X(X-1)\cdots(X-r+1)). $$
%the $r$th (descending) factorial moment of $X$.
%Then we see that for $ r = 0,1,\ldots ,2^L-1$ one has
%\small
%\begin{multline*}
%\mu_{(r)}(X) = \sum_{z=0}^{2^L} (2^L - z)^{(r)} {2^L \choose z}  \sum_{i=0}^{z-1} (-1)^{i} {z \choose i} \left( \frac{z-i}{2^L} \right)^D  = \\
%= (2^L)^{(r)} \sum_{z = 0}^{2^L - r} {2^L - r \choose z} \sum_{i=0}^{z-1} (-1)^{i} {z \choose i} \left( \frac{z-i}{2^L} \right)^D = \\
%= (2^L)^{-D} \cdot (2^L)^{(r)} \sum_{z = 0}^{2^L - r} {2^L - r \choose z} \sum_{i=0}^{z-1} (-1)^{i} {z \choose i} (z - i)^D = \\
%= (2^L)^{-D} \cdot (2^L)^{(r)} (2^L-r)^D = (2^L)^{(r)} \left( 1 - \frac{r}{2^L} \right )^D
%\end{multline*}
%\normalsize
%Of course, $\mu_{(r)}(X) = 0$ for $r \ge 2^L$.
%Therefore, the factorial moment generating function of $X$ is
%\begin{multline*}
%\phi_{X}^{*}(s) = \sum_{j=0}^{2^L} \left( 1 - \frac{j}{2^L} \right)^D \frac{(2^L)^{(j)}}{j!}s^j = \\
%=  \sum_{j=0}^{2^L} {2^L \choose j} \left( 1 - \frac{j}{2^L} \right)^D s^j
%\end{multline*}
%For any $r \ge 0$, denote by $\kappa_r$ the $r$th cumulant. Clearly, for any $r \ge 2$, we have $\kappa_r(Z) = (-1)^r \kappa_r(X)$.
%Introducing the normalized variable $Z' = \frac{Z - \mathbb{E}(Z)}{\sqrt{Var(Z)}}$, we further see that
%\begin{equation} \label{eq:cumulants}
%\kappa_r (Z') = \frac{\kappa_r(Z)}{\sqrt{\kappa_2(Z)}^r} = \frac{(-1)^r}{\sqrt{\kappa_2(X)}^r} \kappa_r(X)
%\end{equation}

%We use the following lemma to continue:
%\begin{lemma}[Lemma 6.2, page 332 of~\cite{Johnson Kotz}]
%For all $r \ge 1$, one has $\kappa_r(X) = O(2^L)$.
%\end{lemma}
%This gives us a good estimate for general values of $r$, but in order to use ~\ref{eq:cumulants} we need a sharper estimate for $\kappa_2(X) = Var(Z)$.
%Luckily, we have Lemma~\ref{lem:DISTINCT variance} and ~\ref{eq:DISTINCT expectation}, so we can calculate exactly $Var(Z) = \mathbb{E}(Z^2) %- (\mathbb{E}(Z))^2)$. In fact, using Corollary~\ref{cor:DISTINCT var approx} we get
%\begin{corollary} \label{cor:DISTINCT variance}
%$Var(Z) \ge \frac{D^3 \varepsilon}{W}$
%\end{corollary}
%\begin{proof}
%Recall that $Var(Z) = \mathbb{E}(Z^2) - (\mathbb{E}Z)^2$.
%By Lemma~\ref{lem:DISTINCT variance}, we have
%\small
%$$ \mathbb{E}(Z^2) = 2^{2L} - \left ( 2^{2L+1} - 2^L \right) \left ( 1 - \frac{1}{2^L} \right)^D +  \left ( 2^{2L} - 2^L \right) \left ( 1 - \frac{1}		%	{2^{L-1}} \right)^D $$\normalsize
%Since
%$$ \mathbb{E}(Z) = 2^L \left( 1 - \frac{1}{2^L}\right)^D $$
%By expanding we see that $Var(Z) = \frac{7}{6} \frac{D^3 \varepsilon}{W} + O \left( \frac{D^4 \varepsilon^2}{W^2} \right)$.
%Observing that the constant in the O notation is negative yields the result.
%\end{proof}

%Therefore, we have
%$$ |\kappa_r(Z')| = O \left( \frac{W}{\varepsilon} \cdot  \frac{W^{r/2}}{D^{3r/2} \varepsilon^{r/2}}  \right)  = O \left( \frac{W^{r/2-1}}{\varepsilon^{r/2}}  \right) $$


%!!! 2DO !!! complete analysis of the marginal probability for DISTINCT2 - either Chernoff-cramer bound and the factorial cumulants. - Considering the %normalized $M_0$ which has cumulants of order $2^{(1-r/2)L}$, use chernoff cramer bound with $s = \beta = \sqrt(2\ln(1\delta))$ and neglect %higher orders by the cumulant bound.
%Now transform this to an inequality on our estimator.
%\textbf{TODO: finish this proof}

\subsection{Analysis of entropy estimation functionality}
\label{anal:entropy}
We now turn to analyze the entropy estimation. 
Recall that SWAMP uses the estimator $\entropyVariable$.
If we denote by $F$ the \text{set} of distinct fingerprints in the last $W$ elements, it is given by
\ifdefined\EXTENDED
$$ \entropyVariable = -\sum_{h \in F} \frac{n_h}{W} \log (\frac{n_h}{W}), $$
\else
$ \entropyVariable = -\sum_{h \in F} \frac{n_h}{W} \log (\frac{n_h}{W}), $
\fi
where $n_h$ is the number of occurrences of fingerprint $h$ in the window of last $W$ elements.
We begin by showing that $\mathbb{E}(\entropyVariable)$ approximates $H$, where
\ifdefined\EXTENDED
$$ H = -\sum_{y \in D} \frac{f_y^W}{W} \logp{\frac{f_y^W}{W}} $$
\else
\\$ H = -\sum_{y \in D} \frac{f_y^W}{W} \logp{\frac{f_y^W}{W}} $
\fi
is the entropy in the window.

\begin{theorem}
	\label{thm:EH}
	$\entropyVariable \le H$ and $\mathbb{E}(\entropyVariable)$ is at least $H -\varepsilon$.
\end{theorem}
\begin{proof}
For any $y \in D$, let $h(y)$ be its fingerprint. Recall that $\widehat{f_y^W}$ is the frequency $n_{h(y)}$ of $h(y)$, hence we have:
\ifdefined\EXTENDED
$$ \widehat{f_y^W} = \sum_{y':h(y)=h(y')} f_{y'}^W. $$
\else
$ \widehat{f_y^W} = \sum_{y':h(y)=h(y')} f_{y'}^W. $
\fi
For ease of notation, we denote $p_y =\frac{f_y^W}{W}$, and  $p_h =  \frac{n_h}{W}$. Thus
\ifdefined\EXTENDED
$$ p_h = \sum_{y \in D:h(y)=h} p_y. $$
\else
$p_h = \sum_{y \in D:h(y)=h} p_y. $
\fi
\\It follows that:
\ifdefined\EXTENDED
\begin{multline*}
\entropyVariable = -\sum_{h \in F} p_h \log(p_h) 
= -\sum_{h \in F} \left(  \sum_{y \in D :h(y)=h} p_y \right) \log \left(  \sum_{y \in D :h(y)=h} p_y \right) 
= -\sum_{y \in D} p_y \cdot \log \left(  \sum_{y' \in D :h(y')=h(y)} p_{y'} \right).
\end{multline*}
\else
{$\entropyVariable = -\sum_{h \in F} p_h \log(p_h)\\
= -\sum_{h \in F} \left(  \sum_{y \in D :h(y)=h} p_y \right) \log \left(  \sum_{y \in D :h(y)=h} p_y \right) \\
= -\sum_{y \in D} p_y \cdot \log \left(  \sum_{y' \in D :h(y')=h(y)} p_{y'} \right).\\
$
}\normalfont
\fi
Now, since $p_{y'} \ge 0$ for all $y'$, it follows that for any $y$,
\ifdefined\EXTENDED
$$ \sum_{y' \in D :h(y')=h(y)} p_{y'} \ge p_y .$$
\else
$ \sum_{y' \in D :h(y')=h(y)} p_{y'} \ge p_y .$
\fi
Hence, by the monotonicity of the logarithm,
\ifdefined\EXTENDED
$$ \entropyVariable \le  -\sum_{y \in D} p_y \log(p_y) = H $$
\else
$ \entropyVariable \le  -\sum_{y \in D} p_y \log(p_y) = H $
\fi
proving the first part of our claim.
Conversely, denote for any $y  \in D$ and any $h \in F$, by $I_{y,h}$ the Bernoulli random variable, attaining the value $1$ if $h(y)=h$. Then we see that:
\ifdefined\EXTENDED
$$ \entropyVariable =  -\sum_{y \in D} p_y \cdot \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right). $$
\else
\\
$ \entropyVariable =  -\sum_{y \in D} p_y \cdot \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right). $
\fi

We see, by using Jensen's inequality, the concavity of the logarithm and the linearity of expectation, that for any $y$:
\small
\ifdefined\EXTENDED
$$ \mathbb{E}  \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right) \le \log  \left(  \sum_{y' \in D} p_{y'} \cdot \mathbb{E}(I_{y',h(y)}) \right) $$\normalsize
\else
$ \mathbb{E}  \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right) \le \log  \left(  \sum_{y' \in D} p_{y'} \cdot \mathbb{E}(I_{y',h(y)}) \right) $
\fi
Since for any $y' \ne y$, we have $ \mathbb{E}(I_{y',h(y)}) = 2^{-L}$, we see that

\small
\ifdefined\EXTENDED
$$ \mathbb{E}  \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right) \le \log  \left( 2^{-L} \cdot \sum_{y' \ne y \in D} p_{y'} + p_y \right) = \log(p_y + 2^{-L}(1-p_y)) $$
\else
$ \mathbb{E}  \log \left(  \sum_{y' \in D} p_{y'} \cdot I_{y',h(y)} \right)\le$$ \log  \left( 2^{-L} \cdot \sum_{y' \ne y \in D} p_{y'} + p_y \right)\\ =  \log(p_y + 2^{-L}(1-p_y)). $
\fi
\normalsize
Summing this over $y$, and using the linearity of expectation once more, we obtain:\\
\ifdefined\EXTENDED
$$ \mathbb{E}(\entropyVariable) \ge - \sum_{y \in D} p_y  \log(p_y + 2^{-L}(1-p_y)). $$
\else
$ \mathbb{E}(\entropyVariable) \ge - \sum_{y \in D} p_y  \log(p_y + 2^{-L}(1-p_y)). $\\
\fi
Subtracting $H$ yields:
\ifdefined\EXTENDED
\begin{align*}
\mathbb{E}(\entropyVariable) - H \ge  -\sum_{y \in D} p_y \left( \log(p_y + 2^{-L}(1-p_y)) - \log(p_y) \right)
\ge - \sum_{y \in D} p_y \left( \log(1 + 2^{-L}(\frac{1}{p_y}-1)) \right).
\end{align*}
\else
{\\
	$\mathbb{E}(\entropyVariable) - H \ge  -\sum_{y \in D} p_y \left( \log(p_y + 2^{-L}(1-p_y)) - \log(p_y) \right)\\
	\ge - \sum_{y \in D} p_y \left( \log(1 + 2^{-L}(\frac{1}{p_y}-1)) \right).
	$
}\normalfont
\fi
\\Note that $2^{-L} = \frac{\varepsilon}{W}$ and $\frac{1}{W} \le p_y < 1$. Hence, $0<2^{-L}(\frac{1}{p_y}-1) < \varepsilon$.
Since for any $0 < x $,  $\log(1+x) < x$, we get:
\ifdefined\EXTENDED
$$ \mathbb{E}(\entropyVariable) - H \ge - \sum_{y \in D} 2^{-L} \cdot (1-p_y) =  - \frac{\varepsilon}{W} \cdot (D - 1).$$
\else
$ \mathbb{E}(\entropyVariable) - H \ge - \sum_{y \in D} 2^{-L} \cdot (1-p_y) =  - \frac{\varepsilon}{W} \cdot (D - 1).$\\
\fi
As $ D \le W $, we get that $  \mathbb{E}(\entropyVariable) > H - \varepsilon $, as claimed.
\end{proof}

We proceed with a confidence interval derivation:
\begin{theorem}\label{thm:entropyInterval}
Let $\epsilon_H = \varepsilon\delta^{-1}$ then $\hat{H}$ solves {\sc $(W,\epsilon_H,\delta)$-Entropy Estimation}. That is:
  $ \Pr \left ( H - \hat{H} \ge \epsilon_H \right ) \le~\delta .$
\end{theorem}
\begin{proof}
Denote by $X\triangleq H - \hat{H}$ the
\ifdefined\EXTENDED
random variable of the
\fi
estimation error. According to Theorem~\ref{thm:EH}, $X$ is non-negative and $E(X)\le \epsilon$.
Therefore, according to Markov's theorem we have
\ifdefined\EXTENDED
\begin{align*}
\Pr \left ( H \le \hat{H} + \epsilon\delta^{-1} \right ) = 1- \Pr \left(  X \ge \epsilon\delta^{-1}  \right) \ge 1- \frac{E(X)}{\epsilon\delta^{-1}} \ge 1- \delta.\quad\qedhere
\end{align*}
\else
{\small
$
\Pr \left ( H \le \hat{H} + \epsilon\delta^{-1} \right ) = 1- \Pr \left(  X \ge \epsilon\delta^{-1}  \right) \ge 1- \frac{E(X)}{\epsilon\delta^{-1}} \ge 1- \delta.\quad\qedhere
$
}\normalfont
\fi
Setting $\epsilon_H = \epsilon\delta^{-1}$
\ifdefined\EXTENDED
and rearranging the expression completes the proof.
\else
concludes the proof.
\fi
\qedhere
\end{proof}

%\begin{figure*}[t]
%	\center{
%		\subfigure[Chicago 16 Dataset]{\includegraphics[width = 5.8cm]{CH16_WCSS_Comparison.png}}
%		\subfigure[Chicago 15 Dataset]{\includegraphics[width = 5.8cm]{CH15_WCSS_Comparison.png}}
%		\subfigure[San Jose 14 Dataset]{\includegraphics[width = 5.8cm]{SJ14_WCSS_Comparison.png}}
%		\subfigure[YouTube Dataset]{\includegraphics[width = 5.8cm]{YouTube_WCSS_Comparison.png}}
%		\subfigure[Datacenter (DC1) Dataset]{\includegraphics[width = 5.8cm]{DC1_WCSS_Comparison.png}}
%		\subfigure[Datacenter (DC2) Dataset]{\includegraphics[width = 5.8cm]{DC2_WCSS_Comparison.png}}
%	}
%	
%	\caption{Space and accuracy trade-off for in estimating per flow packet counts for a window size of $W$.}
%	\label{fig:memWCSS}
%\end{figure*}



==> table_ex.tex <==

 \begin{table*}[t]
	 \footnotesize
 	\addtolength{\tabcolsep}{-0pt} \addtolength{\parskip}{-0.1mm} \center{
 		\begin{tabular}{|c|c|c|c|c|c|}
 			\hline
 			\textbf{Src/Dest } & \textbf{{*}} & \textbf{d1.{*}} & \textbf{d1.d2.{*}} & \textbf{d1.d2.d3.{*}} & \textbf{d1.d2.d3.d4}\tabularnewline
 			\hline
 			\hline
 			\textbf{{*}} & ({*},{*}) & ({*},d1.{*}) & ({*},d1.d2.{*}) & ({*},d1.d2.d3.{*}) & ({*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.{*}} & (s1.{*},{*}) & (s1.{*},d1.{*}) & (s1.{*},d1.d2.{*}) & (s1.{*},d1.d2.d3.{*}) & (s1.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.{*}} & (s1.s2.{*},{*}) & (s1.s2.{*},d1.{*}) & (s1.s2.{*},d1.d2.{*}) & (s1.s2.{*},d1.d2.d3.{*}) & (s1.s2.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.s3.{*}} & (s1.s2.s3.{*},{*}) & (s1.s2.s3.{*},d1.{*}) & (s1.s2.s3.{*},d1.d2.{*}) & (s1.s2.s3.{*},d1.d2.d3.{*}) & (s1.s2.s3.{*},d1.d2.d3.d4)\tabularnewline
 			\hline
 			\textbf{s1.s2.s3.s4} & (s1.s2.s3.s4,{*}) & (s1.s2.s3.s4,d1.{*}) & (s1.s2.s3.s4,d1.d2.{*}) & (s1.s2.s3.s4,d1.d2.d3.{*}) & (s1.s2.s3.s4,d1.d2.d3.d4)\tabularnewline
 			\hline
 		\end{tabular}
 		
 		{{\caption{An example of the lattice induced by a two dimensional source/destination byte hierarchy. The top left corner (*,*) is fully general while the bottom right (s1.s2,s3.s4,d1.d2.d3.d4) is fully specified. The parents of each node are directly above it and directly to the left.}
 				\label{tbl:example}
 			}}}
 		\end{table*}
\normalsize

%\begin{figure}[t]
	
%	\center{
%		\includegraphics[width = \columnwidth]{example.png}
%		\caption{\label{fig:example}An illustration of the lattice induced by byte granularity two dimensional hierarchy. Source ip bytes are denoted a1.a2.a3.a4, while destination bytes are denoted b1.b2.b3.b4. The lattice represents all supported queries for this granularity.
%		}}	
%	\end{figure}


==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
